Evaluating Effectiveness of Interactivity in Contour-based Geospatial Visualizations

Contour maps are an essential tool for exploring spatial features of the terrain, such as distance, directions, and surface gradient among the contour areas. User interactions in contour-based visualizations create approaches to visual analysis that are noticeably different from the perspective of human cognition. As such, various interactive approaches have been introduced to improve system usability and enhance human cognition for complex and large-scale spatial data exploration. However, what user interaction means for contour maps, its purpose, when to leverage, and design primitives have yet to be investigated in the context of analysis tasks. Therefore, further research is needed to better understand and quantify the potentials and benefits offered by user interactions in contour-based geospatial visualizations designed to support analytical tasks. In this paper, we present a contour-based interactive geospatial visualization designed for analytical tasks. We conducted a crowd-sourced user study (N=62) to examine the impact of interactive features on analysis using contour-based geospatial visualizations. Our results show that the interactive features aid in their data analysis and understanding in terms of spatial data extent, map layout, task complexity, and user expertise. Finally, we discuss our findings in-depth, which will serve as guidelines for future design and implementation of interactive features in support of case-specific analytical tasks on contour-based geospatial views.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/0_etc.tex <==

\subsection{Task Specification}\label{sec:task-specification}
We structure this study to provide a data-driven evaluation of whether interactive features in geospatial visualization enhance the performance of exploratory geospatial analysis tasks. In designing the user study, we draw upon the existing literature to identify relevant exploratory analysis tasks for the geo-visualization context. Such tasks often involve identifying clusters, discerning relationships between data points, making comparisons, and analyzing data relevance to specific geographical locations. The literature offers numerous transitions of these tasks into visualization operations \cite{146375, keller1994visual, OGAO200223}. However, these operations can be supported by multiple visual artifacts including geospatial views, parallel coordinates, matrix representations, line plots, and others \cite{koua2006, mayr2018integrated}.

% We review a set of exploratory analysis tasks previously used in evaluating exploratory geovisual environments \cite{keller1994visual, koua2006}. 
% The analysis tasks derived from the selected exploratory task types are common among climate and environmental scientists \cite{koua2006, nayeem2022dcpviz, zahan2021contour, gdlviz2022}. 
% Therefore, this study utilize the exhaustive list proposed by Keller et al. \cite{keller1994visual} and subsequently employed by Koua et al. \cite{koua2006} for a usability study in contour-based exploratory geovisualization. We shape our analytical tasks based on these operations, delineating them into the following seven tasks: 

% \begin{enumerate}[leftmargin=* ]
%     \item \textit{\textbf{Associate}} tasks involve users in finding similarities between data points based on the characteristics of attributes, geographic location, and patterns of events.

%     \item \textit{\textbf{Categorize}} tasks require defining all regions on the display by the boundaries. The regions are usually categorized by common features or spatial positioning.

%     \item \textit{\textbf{Cluster}}-type tasks require users to identify different groups of similar data points or regions within the geospatial data. In these tasks, the user identifies sparse data points or regions that share common attributes to form unique groups within the data.

%     \item \textit{\textbf{Distinguish}} analytical tasks require users to recognize the differences or variations between spatial events. These differences often include the geospatial area or location and values of the same attribute.

%     \item \textit{\textbf{Identify}} tasks demand establishing the relationship between data attributes based on their shared characteristics.

%     \item \textit{\textbf{Locate}} requires recognizing certain data points or events on the map. In this task, we aim to evaluate whether the map supports the user in locating the facts or a range of values.

%     \item \textit{\textbf{Rank}}-type tasks require feature ordering based on data attributes, clusters, or geographic locations.
% \end{enumerate}

% \textit{\textbf{Associate}} tasks involve users in finding similarities between data points based on the characteristics of attributes, geographic location, and patterns of events. \textit{\textbf{Categorize}} tasks require defining all regions on the display by the boundaries. The regions are usually categorized by common features or spatial positioning. \textit{\textbf{Cluster}}-type tasks require users to identify different groups of similar data points or regions within the geospatial data. In these tasks, the user identifies sparse data points or regions that share common attributes to form unique groups within the data. \textit{\textbf{Distinguish}} analytical tasks require the users to recognize the difference or variations between the spatial events. These differences often include geospatial area or location and values of the same attribute. \textit{\textbf{Identify}} tasks demand establishing the relationship between data attributes based on their shared characteristics. \textit{\textbf{Locate}} requires recognizing certain data points or events on the map. In this task, we aim to evaluate whether the map supports the user in locating the facts or a range of values. \textit{\textbf{Rank}}-type tasks require feature ordering based on the data attributes, clusters, or geographic locations.

Exploratory tasks can be categorized based on the number of data points they encompass. These tasks are broadly grouped into simple and complex categories. Simple tasks involve a more direct spatial exploration, primarily focusing on  \textit{distinguish}, \textit{identify}, and \textit{locate} task types. Here, users typically interact with no more than two data points. The essence of these tasks is to either determine the location of a known event or ascertain the event based on its location. 
% and querying the location of where it happened or vice-versa. 
In contrast, complex tasks delve into a deeper spatial analysis, encapsulating \textit{associate}, \textit{categorize}, \textit{cluster}, and \textit{rank} tasks. %type of spatial analysis where the user explore the relationships among multiple data points. 
Here, the exploration revolves around discerning between numerous data points. Users predominantly seek data similarities, often independent of specific locations or events.

For the design of these tasks, we consider both singular and comparative explorations of geospatial data. The synchronized interactions within the map are tailored to aid users in juxtaposing spatial events across multiple maps, a technique prevalent in temporal-spatial data research. While a singular map is adept at providing insights into a specific geospatial instance, our aim is to discern the advantages interactive features confer when analyzing spatiotemporal discrepancies. Consequently, our task designs cater to both individual and multi-map analytical explorations. The comprehensive list of these tasks is presented in Table \ref{tab:exploratory-tasks}. While we acknowledge that the analytical tasks in Table \ref{tab:exploratory-tasks} may span multiple types, we have designated each based on its most dominant analytical characteristic.

%The users generally identify the data similarities and mapping based on a point of interest regardless of location or event. 

% We designed the tasks for each type from the point of view of a single instance of geospatial data exploration and multiple geospatial data comparisons. The synchronize interaction implemented in the map is expected to facilitate the users in comparing the spatial events between multi-maps. Such cases are frequently studied in identifying the temporal changes in spatial data. While the single map obtains the potential to support the exploration of an instance of geospatial data, we intend to measure the support that interactive features provide in analyzing the spatiotemporal differences. Therefore, we designed a set of tasks that account for both single and multi-map analysis and exploratory task types as outlined in Table \ref{tab:exploratory-tasks}. We understand that the analytical tasks in Table \ref{tab:exploratory-tasks} can be related to more than one task type, however, we assigned the type based on the most prominent resemblance of the analysis.


==> sections/5-task-specification__old_.tex <==
\section {Crowd-sourced user study}

Our study design is influenced by a literature review on crowd-sourced studies evaluating visualization components \cite{heer2010, nagel2012, karduni2021} that provided a well-grounded idea on participant recruitment and exclusion criteria, training requirements and study procedures. 




\subsection{Participants \& Recruitment}
\begin{figure}[t]
    \centering

    \includegraphics[width=0.9\linewidth]{figures/demographic-summary.png}
    \caption{Summary of 62 participants' educational qualifications, computer usage, geospatial expertise, and visualization expertise. }
    \label{fig:demographic-data}
\end{figure}
We host the study online, with participants sourced from Amazon Mechanical Turk (MTurk). Our user study interface is directly linked to a Human Intelligent Task (HIT) we posted on the MTurk portal. 
To ensure the quality of the collected data, we selected participants from MTurk who had an approval rating above 95\% and were identified as master workers. \HDY{We initially recruited a total of 67 participants, all based in the United States.}
In line with our pre-registration criteria, we excluded four participants who failed engagement questions and another one participant who completed the study in under 8 minutes. This led to a final sample size of 62 participants (25 females and 37 males). 
We asked the participants about their academic qualifications, their daily computer usage, and how they rate their expertise in perceiving visualization and analyzing geospatial data. 
For computer usage, visualization expertise, and geospatial analysis expertise, the participants identify themselves from the groups shown in Fig. \ref{fig:demographic-data}. 
They identified themselves as having various levels of expertise in visualization and geospatial analysis (Fig. \ref{fig:demographic-data}). 
Each participant earned a \$4 incentive for their contribution to our user study.
On average, they took 8.6 minutes (\textit{SD=7.99}) for the training session and 29.14 minutes (\textit{SD=19.75}) to complete the main session.




==> sections/6-user-study__old_.tex <==

\subsection{Study Factors}


\subsubsection{Map Type}

In this work, we divide map types into two categories: static map (Fig. \ref{fig:interaction-teaser}A) and interactive map (Fig. \ref{fig:interaction-teaser}B), based on their level of interactivity. The interactive map supports the aforementioned interactive features. 
Please keep in mind that the interactive map provides all the features, and we do not exclude or omit any specific features.  We made this decision to ascertain and discuss which interactive features participants commonly utilize to accomplish the tasks. Conversely, the static map is designed considering the traditional approach of contour maps and only offers panning and zooming capabilities.

\subsubsection{Map Layout}\label{section_map_layout}
The map layout includes two conditions: single map and multiple map. The single map condition provides only one static or interactive map, as the name implies. The multiple map displays two maps side by side, with each map potentially containing data from different locations or time periods. We refer to them as Snapshot Left/Right. They are either static or interactive maps.



\bgroup
\def\arraystretch{1.2}%
\begin{table*}[h]
\centering
\caption{The participants performed \HDY{these geovisual analyses} from seven unique task types. \HDY{These tasks} are designed for both single and multiple map layouts to evaluate the usability of interactive features in a geovisual environment.
% The participants performed these exploratory geovisual analyses from seven unique task types. These exploratory tasks are designed for both single and multiple map layouts to evaluate the usability of interactive features in a geovisual environment.
}
\begin{tabular}{| p {5em}| p {24em} | p{25em} |}
\hline
\textbf{Task Type} & \textbf{Single Map}                                                                                                                                                                                          & \textbf{Multiple Map}                                                                                                                                                                            \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Associate          & Based on the area covered which two \emph{[variable/marker]} intensities below are the most similar?                                                                                    & Find the \emph{[variable/marker]} intensities from both snapshot that cover the \emph{[largest/smallest]} area.                                        \\ \hline
Categorize         & What is the \emph{[area/intensity]} (difference) for the \emph{[highest intensity/largest area]} recorded on \emph{[contour/Location X]}? & What is the area difference of \emph{[variable]} \emph{[intensity]} between Snapshot Left and Right?                                                   \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Cluster            & How many \emph{[unique/total]} contour regions are visible on the map?                                                                                                                  & How has the number of \emph{[unique/total]} contour regions changed from `Snapshot Left' to `Snapshot Right'?                                                               \\ \hline
Distinguish        & What is the \emph{[area/intensity]} difference between the highest and lowest \emph{[variable]}?                                                                   & How does the \emph{[highest/lowest]} intensity shift from `Snapshot Left' to `Snapshot Right'?                                                                              \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Identify           & What is the \emph{[intensity/difference between]} \emph{[variable]} in Location \emph{[X]} (and Location \emph{[Y]})?    & What is the intensity difference between Location \emph{[X]} in `Snapshot Left' and Location \emph{[Y]} in `Snapshot Right'?                           \\ \hline
Locate             & What is the \emph{[highest/lowest]} intensity on the \emph{[contour/marked area]}?                                                                                 & What is the \emph{[highest/lowest]} intensity \emph{[between both snapshots/among all markers]}?                                                       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Rank               & Order the \emph{[markers/intensities below]} from \emph{[high to low/low to high]} \emph{[intensity/area]}.                                   & Order the snapshots based on the \emph{[larger/smaller]} area covered by the \emph{[lowest/highest]} \emph{[variable]} intensity. \\ \hline
\end{tabular}
\label{tab:exploratory-tasks}
\vspace{-.3cm}
\end{table*}

% \subsubsection{Exploratory Tasks}
\subsubsection{\HDY{Visualization Analysis Tasks}}
% In this work, we consider the seven visual exploratory tasks identified in Section~\ref{sec:visual-tasks}. 
This work considers the seven \HDY{visualization tasks} identified in Section~\ref{sec:visual-tasks}. 
% \HDY{These tasks} can be categorized based on the number of data points they encompass. These tasks are broadly grouped into simple and complex tasks. 
\HDY{These tasks} can be broadly categorized as simple or complex tasks, depending on the number of data points they encompass.
Simple tasks involve a more direct spatial exploration, primarily focusing on  \textit{distinguish}, \textit{identify}, and \textit{locate} task types. Here, users typically interact with no more than two data points. The essence of these tasks is to either determine the location of a known event or ascertain the event based on its location. 
In contrast, complex tasks delve into a deeper spatial analysis, encapsulating \textit{associate}, \textit{categorize}, \textit{cluster}, and \textit{rank} tasks. 
Here, the exploration revolves around discerning between numerous data points. Users predominantly seek data similarities, often independent of specific locations or events.

For the design of these tasks, we consider both singular and comparative explorations of geospatial data. The synchronized interactions within the map are tailored to aid users in juxtaposing events across multiple maps, a technique prevalent in temporal-spatial data research. While a singular map is adept at providing insights into a specific geospatial event, our aim is to discern the advantages interactive features confer when analyzing spatiotemporal discrepancies. Consequently, our task designs cater to both individual and multi-map analytical explorations. 
The comprehensive list of these tasks is presented in Table \ref{tab:exploratory-tasks}. 
Please refer to the supplementary materials for a complete list of questions.
While we acknowledge that the analytical tasks in Table \ref{tab:exploratory-tasks} may span multiple types, we have designated each based on its most dominant analytical characteristic. \placeholder{It is worth noting that due to the inherent differences between single- and multi-map layouts, the questions within each task are not identical.  
However, the questions are comparable to the given task types in order to assess the effectiveness of each layout. 
Therefore, we chose to use the map layout as the primary variable in order to isolate and evaluate its influence on different task types.
% However, to assess the effectiveness of each layout, we decided to use the map layout as a primary variable to isolate and evaluate how the layout influences task completion.
This approach could provide valuable information on how different layouts influence user performance, even with variations in task questions.
}
These tasks involve multiple-choice questions, where participants select one correct answer from three options. 


\subsubsection{Others}
\hspace{\parindent}\textbf{Map Data Context:}
To examine the general effect of interactive features, two datasets with different spatial ranges are utilized in this study (i.e., NY Temperature and CONUS Precipitation).
On one hand, NY Temperature provides temperature data (D\textsubscript{T}) for a limited spatial extent around New York. 
On the other hand, CONUS Precipitation provides precipitation data (D\textsubscript{P}) for the contiguous U.S., covering a larger area than \textit{NY Temperature}.
The numbers following D\textsubscript{T} and D\textsubscript{P} in Table~\ref{tab:task-distribution} refer to the distinct subsets of data. The seven questions for the multi map task sets in Table \ref{tab:exploratory-tasks} are developed using the two datasets separately. 
 


\textbf{Participants' Expertise:} We consider the participants into two groups - novice and experienced, based on their reported expertise in geospatial analysis. 
The participants who identified themselves as \textit{`unfamiliar'} or \textit{`somewhat familiar'} with geospatial analysis are classified as novice users, and the other participants who identified themselves as \textit{`somewhat experienced'}, \textit{`experienced'}, or \textit{`expert'} are classified as experienced users. 
The sample ratio between these two groups was 1.06 which is fairly equal, as Fig. \ref{fig:demographic-data} suggests.





% \bgroup
% \def\arraystretch{1.2}%
\begin{table}[t]
% \small
\centering
\caption{Distribution of the 8 sets of tasks that account for the repetitive measures such as the spatial extent, visualization methods, and map layout. Each task set includes a task from the classification of \HDY{the analysis tasks.}
% Each task set includes a task from the classification of the exploratory analysis tasks.
}
% \begin{tabularx}{|c|l|c|c|}
% \begin{tabularx}{\columnwidth}{|X|X|X|X|}
\scriptsize
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{tabular} {P{2.5cm} | P{2.6cm} | P{1.1cm}| P{1.1cm}}
\hline
\textbf{Map Data Context} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Map Data\\ (Task Set)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Participant\\ Group 1\end{tabular}}                          & \textbf{\begin{tabular}[c]{@{}c@{}}Participant\\ Group 2\end{tabular}}                          \\ \hline
                                                                                                                              & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{T}1                                                                             & \cellcolor[HTML]{EFEFEF}                                                                         &                                                                                                 \\ 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Small Spatial Extent\\ (NY Temperature)\end{tabular}}                             & Multi Map - {[}D\textsubscript{T}2, D\textsubscript{T}3{]}                                                                    & \cellcolor[HTML]{EFEFEF}                                                                         &                                                                                                 \\ \cline{1-2}
\cellcolor[HTML]{EFEFEF}                                                                                                      & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{P}1                                                                             & \cellcolor[HTML]{EFEFEF}                                                                         &                                                                                                 \\ 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Large Spatial Extent\\ (CONUS Precipitation)\end{tabular}} & Multi Map - {[}D\textsubscript{P}2, D\textsubscript{P}3{]}                                                                    & \multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Static\\Maps\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Interactive\\Maps\end{tabular}}                    \\ \cline{1-2}
                                                                                                                              & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{T}4                                                                             &                                                                                                  & \cellcolor[HTML]{EFEFEF}                                                                        \\ 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Small Spatial Extent\\ (NY Temperature)\end{tabular}}                             & Multi Map - {[}D\textsubscript{T}5, D\textsubscript{T}6{]}                                                                    &                                                                                                  & \cellcolor[HTML]{EFEFEF}                                                                        \\ \cline{1-2}
\cellcolor[HTML]{EFEFEF}                                                                                                      & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{P}4                                                                             &                                                                                                  & \cellcolor[HTML]{EFEFEF}                                                                        \\
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Large Spatial Extent\\ (CONUS Precipitation)\end{tabular}} & Multi Map - {[}D\textsubscript{P}5, D\textsubscript{P}6{]}                                                                    & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Interactive\\Maps\end{tabular}}   & \multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Static\\Maps\end{tabular}} \\ \hline
\end{tabular}
\label{tab:task-distribution}
\end{table}



\subsection{Procedure}

Upon accessing the interface, the participants are first presented with an overview of the study, detailing the procedure, assignments, and the type of interaction data to be captured, culminating in a request for their consent. Subsequently, the interface collects basic demographic information from the participants such as level of education, gender, expertise with geospatial data analysis, familiarity with data visualization, and daily computer usage. 
The participants are then transitioned to a training session that introduces the interactive features for the purpose of visual exploration. 
Across its 12 sections, the training modules elucidate the nuances of the contour map, the geospatial data, and the available interactive elements. To ensure comprehension, the participants encounter sample questions post each interactive feature's detailed explanation. 
Incorrect answers are met with on-screen guidance leading them to the correct response.
This feedback mechanism is unique to the training phase and is deactivated during the main session. 
Upon training completion, they are seamlessly moved to the main study session.  


In the main study session, the participants encounter 8 task sets (i.e., the second column in Table \ref{tab:task-distribution}), split into two distinct sections. Each set corresponds to a map layout showcasing different geospatial data. Within each set, there is a question representing each of the seven task types, culminating in a total of 56 questions (eight task sets $\times$ seven task questions) throughout the study. 
Table \ref{tab:task-distribution} provides a fair distribution of the map and task types, ensuring samples are counterbalanced and repetitive measures are taken into account. 
The tasks are multiple choice type questions regarding the questions in Table~\ref{tab:exploratory-tasks}, and the participants can submit their answer by selecting from the options provided for each task. As participants perform the tasks, either by interacting or observing the map visualization, the interface logs their observations, task completion time (in seconds), and usage of any interactive features associated with questions. Upon completing the study, They get a completion code from the interface. They then submit the code to the MTurk portal to claim their incentive.





\subsection{Evaluation Metrics}
Evaluating geospatial visualizations involves both qualitative and quantitative metrics \cite{tominski2011information}. 
In our study, we focus on quantitative metrics to evaluate the efficacy of interactive features embedded within the contour map. 
Roth \cite{roth2013empirically} described the objectives of cartographic interaction, to name a few, as (1) presenting insights preemptively, (2) coming to a decision point faster, meaning not solely doing it with a visual inspection. 
% To assess the effectiveness of the interactive features \HDY{in analysis tasks} and validate our hypotheses, we focus on the  quantifiable factors - \textit{\textbf{task completion time}} and \textit{\textbf{the accuracy of their \HDY{performed task} -}} and \textit{\textbf{interaction logs during the task}}. 
To assess the effectiveness of the interactive features \HDY{in analysis tasks} and validate our hypotheses, we focus on the  quantifiable factors - \textit{\textbf{the task accuracy and \textit{\textbf{completion time} of their \HDY{performed task}}} -} and \textit{\textbf{interaction logs during the task}}. 
% To assess the effectiveness of the interactive features in exploratory analysis tasks and validate our hypotheses, we focus on the  quantifiable factors - \textit{\textbf{task completion time}} and \textit{\textbf{the accuracy of their performed exploratory task -}} and \textit{\textbf{interaction logs during the task}}. 
The accuracy measures the participant's analytical ability to correctly answer the given multiple-choice questions. \placeholder{Each study condition includes three questions, and task accuracy is calculated based on the number of correct answers. While the the task accuracy is 
 inherently a continuous value, only three discrete values of accuracy are available (0 (0\%), 1 (50\%), and 2 (100\%)).% (\%) reflecting percentage-based task accuracy (see the supplemental material). 0 indicates complete failure, 50 indicates partial accuracy, and 100 indicates full accuracy.
 We consider that the intervals between these scores (0 to 50 and 50 to 100) reflect equal changes in task performance. 
Despite the discrete nature of these values, %As a result, 
we treat accuracy as a continuous variable~\cite{robitzsch2020ordinal}, given that the scores are proportional and reflect distinct performance levels on an underlying continuous scale of task accuracy. Therefore, we use continuous analysis methods, as outlined in Section ~\ref{section-result}.
% In this work, we approximate this as a continuous variable, as the scores are proportional and represent distinct levels of performance on an underlying continuous scale of task accuracy. 
% While the values are discretized into three values for simplicity, we assume that the intervals between these scores (0 to 50 and 50 to 100) reflect equal changes in task performance, justifying the use of continuous analysis methods in Section~\ref{section-result}.
}


\subsection{Hypotheses} \label{sec:hypothesis-rq}

Acknowledging the potential of interactive contours in a geospatial view for visually analyzing geospatial data, it is essential to understand the utility of interactive features to the full extent. 
To address our RQs in Section 1, we establish the following hypotheses for our study:


    \begin{enumerate}[label=\textbf{H\arabic*:}]
    % \item Interactive features can improve users' accuracy when performing exploratory geospatial analysis tasks. 
    \item Interactive features can improve users' accuracy when \HDY{performing geospatial} analysis tasks. 
    
    \item When the interactive features are available, users might need more time to complete tasks \HDY{compared to using} the static map due to associated cognitive processing.
    

    \item When two maps are presented, interactive features of synchronization could offer the potential to improve accuracy in multiple map exploration tasks. 

    

\end{enumerate}




==> sections/7-results__old_.tex <==
\section{Results}\label{section-result}

We leverage two-way repeated measures analysis of variance (ANOVA) at a 95\% confidence level. It evaluates performance metrics based on the map types (interactive vs. static) and map layouts (single map vs. multi map) across the task types. Although our results violate the normality test, we use ANOVA because the previous study~\cite{blanca2017non} provided empirical evidence for its robustness when evaluating data with non-normal distributions. To present the estimates, we also report the lower and upper bounds at a 95\% confidence interval (CI). To present differences between visualization methods, we report the $p$-value and the error bound mean ($EBM$) for the task types. 

\subsection{Accuracy}

Fig. \ref{fig:performance-ci} shows the accuracy results by task types, and map types and layouts. 


\hspace{\parindent}\textbf{Associate:} 
Main effects of map type ($p<.001$, $F(1, 61)=24.362$, $\eta^2_p=.285$) and layout ($p=.017$, $F(1, 61)=6.015$, $\eta^2_p=.090$) were disclosed. The task accuracy suggests that the participants performed substantially better using the interactive map ($M=.460$, $EBM=[.403, .516]$) compared to the static map ($M=.294$, $EBM=[.247, .341]$). We also find the participants performed the task more accurately when they used multi-map ($M=.431$, $EBM=[.367, .500]$) than the single-map ($M=.323$, $EBM=[.268, .377]$).


\textbf{Categorize:} 
We found main effects of map type ($p<.001$, $F(1, 61)=13.897$, $\eta^2_p=.186$) and map layout ($p<.001$, $F(1, 61)=13.346$, $\eta^2_p=.180$). \HDY{The accuracy when using the interactive map ($M = .581$, $EBM = [.509, .652]$) is statistically higher than when using the static map ($M = .431$, $EBM = [.376, .487]$) for categorize-type tasks.}
Next, the multi-map condition ($M=.581$, $EBM=[.518, .643]$) showed higher accuracy than the single-map condition ($M=.431$, $EBM=[.365, .498]$).


\textbf{Cluster:} The map type ($p<.001$, $F(1, 61)=19.973$, $\eta^2_p=.247$) and map layout ($p=.036$, $F(1, 61)=4.611$, $\eta^2_p=.070$) showed main effects. 
Regarding the map type, its pairwise comparison result shows that the interactive map ($M=.560$, $EBM=[.491, .630]$) supported the participants better than the static map ($M=.363$, $EBM= [.297, .429]$). The multi-map condition ($M=.520$, $EBM=[.455, .585]$) showed higher accuracy than the single-map condition ($M=.403$, $EBM=[.320, .486]$).


\textbf{Distinguish:} An interaction effect between the map type and layout was found ($p=.015$, $F(1, 61)=6.295$, $\eta^2_p=.094$). We found a simple effect of the map type when the map layout is multi-map ($p=.002$, $F(1, 61)=10.738$, $\eta^2_p=.150$). Its post-hoc test showed the interactive map ($M=.629$, $EBM=[.553, .705]$) has higher accuracy than the static map ($M=.444$, $EBM=[.354, .533]$).

We found a main effect of map layout ($p=.022$, $F(1, 61)=5.544$, $\eta^2_p=.083$) but not map type ($p=.117$, $F(1, 61)=2.531$, $\eta^2_p=.040$). The pairwise comparison showed the multi-map condition ($M=.536$, $EBM=[.476, .597]$) showed higher accuracy than the single-map condition ($M=.435$, $EBM=[.372, .499]$).


\textbf{Identify:} 
Main effects of map type ($p=.030$, $F(1, 61)=4.923$, $\eta^2_p=.075$) and map layout ($p<.001$, $F(1, 61)=12.219$, $\eta^2_p=.167$) were revealed. The posthoc test revealed \HDY{that} the participants achieved better results with the interactive map ($M=.516$, $EBM=[.444, .588]$) compared to the static map ($M=.415$, $EBM=[.355, .476]$). It also found the participant with the single-map condition ($M=.544$, $EBM=[.480, .609]$) had higher accuracy than the multi-map condition ($M=.387$, $EBM=[.319, .455]$).


\begin{figure}[t]
    \centering
   
    \includegraphics[width=\linewidth]{figures/accuracy-result-2024-2.png}
    \caption{
    The accuracy results by tasks, map types, and map layouts}
    \label{fig:performance-ci}
    % \vspace{-.5cm}
\end{figure}
\textbf{Locate:} We only found a main effect of map layout ($p=.002$, $F(1, 61)=10.333$, $\eta^2_p=.145$). Its pairwise comparison showed the multi-map condition ($M=.835$, $EBM=[.767, .903]$) showed higher accuracy than the single-map condition ($M=.710$, $EBM=[.643, .776]$).


\textbf{Rank:} We discovered the main effects of map type ($p=.003$, $F(1, 61)=9.445$, $\eta^2_p=.134$) and map layout ($p<.001$, $F(1, 61)=15485$, $\eta^2_p=.202$).
The interactive map ($M=.730$, $EBM=[.669, .791]$) has a higher accuracy than the static map ($M=.597$, $EBM=[.527, .667]$). The single-map ($M=.722$, $EBM=[.668, .776]$) has a higher accuracy than the multi-map ($M=.605$, $EBM=[.543, .666]$).


\subsection{Task Completion Time}
Fig. \ref{fig:single-multiple-performance-ci} shows the task completion time results by task types, and map types and layouts. 

\hspace{\parindent}\textbf{Associate:} We found no interaction effect ($p=.102$, $F(1, 61)=2.761$, $\eta^2_p=.043$), but found main effects of map type ($p=.016$, $F(1, 61)=6.091$, $\eta^2_p=.091$) and map layout ($p=.019$, $F(1, 61)=5.849$, $\eta^2_p=.087$). 
The pairwise comparison results for the map type showed the participants spent statistically more time on the interactive map ($M=62.188s$, $EBM=[45.547, 78.829]$) than the static map ($M=45.535s$, $EBM=[34.210, 56.859]$). Next, we also found the participants spent more time on the multi-map condition ($M=60.175s$, $EBM=[45.053, 75.298]$) than single-map ($M=47.547s$, $EBM=[35.716, 59.378]$).


\textbf{Categorize:} We found a main effect of map type ($p=.005$, $F(1, 61)=8.480$, $\eta^2_p=.122$). Its pairwise comparison disclosed that the interactive map condition ($M=98.020s$, $EBM=[74.024, 122.017]$) takes more time than the static map condition ($M=69.519s$, $EBM=[55.645, 83.392]$). 



\textbf{Distinguish:} A main effect of map layout ($p=.026$, $F(1, 61)=5.236$, $\eta^2_p=.079$) was reported. Its pairwise comparison disclosed that the single-map condition ($M=47.473s$, $EBM=[37.381, 57.565]$) takes more time than the multi-map condition ($M=38.201s$, $EBM=[29.710, 46.692]$). 

\textbf{Identify:} The task completion time difference is statistically significant between the map types ($p=.023$). The participants spent more time in the interactive map condition ($M=58.340s$, $EBM=[45.385, 71.296]$) than the static map condition ($M=47.859s$, $EBM=[36.327,59.392]$).

\textbf{Cluster, Locate, \& Rank:} No clear difference in task completion time is disclosed by the task type and layout.





\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/taskCompletionTime-result-2024-2.png}
    \caption{
    The task completion time results by tasks, map types, and map layouts 
    }
    \label{fig:single-multiple-performance-ci}
\end{figure}




==> sections/8-discussion__old_.tex <==
% diagnostic analysis in discussion section
\section{Discussion}


Our user study results partially support all hypotheses. 
In response to \textbf{RQ1}, we found that the results partially support \textbf{H1} and \textbf{H3}. The accuracy was significantly improved by the interactive features for five out of seven tasks (i.e., Associate, Categorize, Cluster, Identify, and Rank). These results align with the perspectives of both DiBiase \cite{dibiase1990visualization} and Roth \cite{roth2008addressing}, indicating that user interaction, particularly in terms of precision performance, aids in uncovering data relationships. However, we found no clear evidence that introducing interactivity improves task accuracy for Distinguish and Locate.  We also found that multi-map is helpful for the Associate, Categorize, Cluster, Distinguish and Locate tasks. 
However, single-map showed better performance in the Identify and Rank tasks compared to multi-map. 

Additionally, the results partially support \textbf{H2}. Despite the performance enhancements offered by the interactive features, we observed no noticeable variation in completion time for the Cluster and Rank tasks. However, the Associate, Categorize, and Identity tasks exhibited longer durations. 
In the following section, we explore RQ1 more thoroughly by examining the impact of participant expertise. We then proceed to analyze RQ2, drawing upon the insights gleaned from our study.








\subsection{Observations from the User Interaction Logs}
% To better understand participants' usage and pattern of interaction features, we examine interaction logs within the context of the exploratory analysis task types.
To better understand participants' usage and pattern of interaction features, we examine interaction logs within the context of \HDY{the analysis task types}.
We classify the interactions based on the number of mouse/keyboard operations (steps) required to perform the feature. Following that, we eliminate unintended interactions in the process of aggregating their interaction logs.
For instance, despite participants only needing to move the cursor to inspect contour regions, they unintentionally interacted with other contour areas while navigating towards deeper parts of the map.
We filter out these unintended interactions by using a time threshold, focusing on areas where participants spent a notable duration, suggesting they were genuinely processing the information displayed on tooltips or widgets.
Fig. \ref{fig:interaction-usage} shows a comprehensive overview of the usage patterns for the interactive features except for synchronization.


\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[width=\linewidth]{figures/interaction-usage-dy.png}
    \caption{
    % The frequently used interactive features in the participating exploratory tasks. 
    The frequently used interactive features in the \HDY{participating tasks.}
    The plotted range of usage frequency is categorized by the task types and bootstrapped with a 95\% confidence interval.
    }
    \label{fig:interaction-usage}
\end{figure}

\textbf{Identifying the frequently used interactive features:} 
We find that inspection and selection are the most frequently used functions, followed by annotation, filter/search, and encode. 
First of all, we observe that the participants frequently inspected or selected various distinct contour regions during the tasks involving association, categorization, and clustering. We expect that they used these interactive features to understand the relationships among different intensity levels.



Next, annotations are mostly used in the locate, rank, and associate tasks. 
It is particularly useful in the rank task because the marker widget provides insights for comparison with other annotations, thereby aiding in determining the order of the contour regions. We also observe that the annotation interaction generally comes after the inspection, selection, and filter interactions.

The filter interaction is frequently utilized in the identify and categorize tasks, often involving searching based on geolocation. 
The identify tasks require to extract information based on geographical characteristics. Thus, participants used the search feature to annotate or inspect intensities according to the locations. The comparative information provided by the annotated locations is continuously updated as the participants interact with other contour regions providing effective categorization and clustering tasks, which involve identifying the regions with similar variability.


At last, we identify that the encoding feature is mostly used in the cluster and identify tasks. The contour encodings are understandably useful in the cluster tasks, as it is often required to identify the unique regions on the contour map. The identify tasks involve the geographical characteristics that usually reside in the base map, hence, the participants' controlled styles correlate with the contour map in these tasks. Therefore, changing the weight and opacity of the contour lines and region's area can be beneficial in visually performing these tasks.


\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[width=\linewidth]{figures/interaction-pattern-dy2.png}
    \caption{Task-wise user interaction pattern based on the normalized task completion time window. The highlighted area represents the time segments where participants' interactivity exceeds the mean.}
    \label{fig:interaction-pattern}
\end{figure}

\textbf{Reflecting cognitive process with interaction usage:}
Fig. \ref{fig:interaction-pattern} presents the number of user interaction usage over time. We normalize the time based on task completion time for each task.
It provides the opportunity to estimate the segments where the participants are seemingly cognitively active. 
Red lines represent the average number of user interaction usage, and highlighted areas show the windows where participants' interactivity exceeds the average. 
The periods of inactivity, particularly at the beginning and end, reflect participants' cognitive processing as they attempted to comprehend the task at hand, plan their next move, or reach an analytical conclusion. 


The average numbers of user interaction usage by the tasks reveal that the participants were especially interactive during more complex tasks such as associating, categorizing, and ranking. 
They also devoted significant time to cognitively processing relationships between spatial data points.
In contrast, for tasks such as distinguishing and locating, participants were notably less interactive. 
This pattern is further reflected in the accuracy score, where the performance disparity between static and interactive maps is minimal for these specific tasks.


\subsection{Performance Elevation by Geospatial Expertise}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/performance-by-user-expertise-dy.png}
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Comparison between novice and experienced participants' performance suggests that novice users excel with interactive features significantly more than experienced users.
    \HDY{The X-axis represents user performance, measured as the total number of correct answers divided by the total task completion time.}
    }
    \label{fig:user-performance-by-expertise}
\end{figure*}


Our results show that the interactive map could improve the novice users' performance when compared to the static map, closing performance gaps between novice and experienced.
This is because interpreting information on a static map typically demands a certain level of expertise, whereas interactive maps have the potential to facilitate a better understanding for both expert and novice users alike. 
We examine the participants' accurate task completion per unit of time in the \HDY{seven analysis} task types. 
% We examine the participants' accurate task completion per unit of time in the seven exploratory analysis task types. 
It is calculated by total number of correct answers by the total amount of task completion time. 
Fig. \ref{fig:user-performance-by-expertise} illustrates task-wise density plots to separately compare the performance measures of both novice and experienced users in interactive and static maps respectively. 
The dashed lines in Fig. \ref{fig:user-performance-by-expertise} represent the performance mean for static (gray) and interactive (green) maps. 
It shows that experienced users performed significantly better than novice users. 
It also shows that the interactive features improved novice users' performance in the associate, cluster, and rank tasks more than experienced users.
At the same time, however, the results reveal that the categorization task is found to be particularly difficult for novice users compared to the other tasks.

 \subsection{Design Considerations for Interactive Contour Map}
\begin{itemize}
    \item \textbf{Prioritize Interactive Features:} Emphasize the development and improvement of interactive features.
    Such features significantly influence users' analytical performance.

    \item \textbf{Consider User Expertise:} It is important to understand how performance varies with the expertise levels of end-users. Interactive maps can be particularly helpful for novice users, effectively bridging the performance gaps seen with traditional static maps.

    \item \textbf{Address Interaction Efficiency:} It is crucial to note that while interactive maps may improve accuracy, they might also increase task completion time. It is important to refine the efficiency of interactive features to ensure a balance between accuracy and time efficiency.

    \item \textbf{Tailor Interactions to Task Types:} Interactive features should be customized based on \HDY{the analysis task types}. 
    % Interactive features should be customized based on the exploratory task types. 
    For instance, emphasize inspection and selection for single-step interactions and consider multi-step interactions for tasks such as locating.
    In addition, the value of annotations, especially in tasks involving ranking and associating cannot be overstated. Users should be encouraged to engage with annotations after inspection, selection, and filter interactions to help their decision-making process.
    

\end{itemize}

\subsection{Future Work}
% \placeholder{We considered the accuracy measurement as a continuous variable in the assumption that the accuracy intervals represent equal changes in task performance. However, this may not fully capture the underlying continuous nature of the performance. 
% Future research should include a larger number of multiple-choice questions with extended study time to gain deeper insights into user performance. }

In this work, we found that interactive features could significantly improve correctness in geospatial data exploration tasks. However, we observed that the participants struggled in \HDY{complex analysis tasks} such as the associate, categorize, and cluster tasks which require in-depth spatial correlation and comparison compared to the simple identify and locate tasks. 
% However, we observed that the participants struggled in complex exploratory tasks such as the associate, categorize, and cluster tasks which require in-depth spatial correlation and comparison compared to the simple identify and locate tasks.
Additionally, the overall correctness for the tasks is less than 70\%, indicating that the navigation task accuracy still needs to be improved.
Interactive features can effectively support users in data exploration beyond individual visualization elements by facilitating coordinated interactions among different visual components.
In our future research, we aim to investigate visualization components which could support the interactive map view and the benefits of coordinated interaction between them. 
It also involves evaluating visualization approaches with various domain-specific experts in geographic spatial analysis, identifying their key tasks within each domain and evaluating interactive features that effectively support their tasks in terms of both quantitative and qualitative assessments.

==> sections/Prev/1-introduction.tex <==
% (-) Poor justification regarding various choices of the study (R1, R2)
% (-) Lack of connection with real domain use cases (R1)
% (-) The main topic being addressed (impact of interaction) was already well studied in previous works, and the paper does not provide new compelling results (R1, R4)
% (-) Lack of detailed description regarding the different comparisons made in the study (R2, R4)
% (-) The design of the experiment does not allow for a more nuanced comparison between different interactive features (R3)
% (-) Problems with the figures (R3, R4)

% \section{Introduction}
% start with geospatial and build on contour map

\section{Introduction}
\maketitle
\label{sec_introduction}
% ***WHEN SCRAPPING ANYTHING IN THIS SECTION, PLEASE MAKE SURE THE CONTEXT FOR THE DATASET USED, INTERACTION FEATURES, EXPLORATORY TASKS, AND THE STUDY MOTIVES ARE NOT BEING REMOVED.***
\IEEEPARstart{G}{eospatial} 
visualizations have become indispensable tools for supporting the analysis of spatial variables across a wide range of research domains, including atmospheric science \cite{McLean2020, Alder2015, li2020sovas}, meteorology \cite{wang2014, Sharma2018, wang2019open}, and urban planning \cite{8613864, zeng2014visualizing, feng2020topology}. 
% Contour maps, a traditional cornerstone of geospatial visualizations, enable the complex analysis of geographical phenomena such as landform shapes, mountain elevations, ocean depths, and climate projections. 
Contour maps, a traditional cornerstone of geospatial visualizations, enable a complex analysis of geographical events (hereafter referred to as ``events''). These events include atmospheric and meteorological phenomena, such as landform shapes, mountain elevations, ocean depths, and climate projections. 
In recent years, collaboration between visualization researchers and domain experts has intensified, leading to multidisciplinary research. These collaborative efforts have been instrumental in developing effective geovisualizations and interaction techniques to identify hidden patterns \cite{Steed2020, nayeem2021visual, maceachren1997exploratory, andrienko2007geo, andrienko2007geo, robinson2017}. However, compared to other forms of geovisualizations such as Choropleth \cite{andrienko2001choropleth} and Cartogram \cite{nusrat2016state}, the exploration and interaction potential of contour maps has not been fully realized. 
% These alternative visualization types demonstrate how user interactions can significantly enhance data analysis, underscoring the under-explored potential of contour maps.

% Our literature review \cite{tominski2011information, afzal2019state, CHEN2019129, andrienko2020spatio} and collaborations within the earth sciences domain reveal that many domain experts rely on traditional static depictions of geospatial data in contour visualizations to perform common visual analysis tasks \cite{gibson2017use, Lee2014}. 
Earlier research \cite{tominski2011information, afzal2019state, CHEN2019129, andrienko2020spatio, nayeem2022dcpviz, gdlviz2022} indicates that many domain experts rely on traditional static depictions of geospatial data in contour visualizations \cite{gibson2017use, Lee2014}. 
% As the spatial resolution of climate projection models improves, their performance typically enhances, providing better representations of extreme weather events \cite{Lee2014}, the hydrological cycle \cite{Lee2017}, and influential land surface processes \cite{DeSales2013}. 
Recently, improved spatial resolution in climate projection models leads to better representations of extreme weather events \cite{Lee2014}, the hydrological cycle \cite{Lee2017}, and important land surface processes \cite{DeSales2013}.
Although contour maps can present 3D information in 2D space and provide a topographic view, they have limitations when dealing with finer spatial resolution data \cite{nayeem2022dcpviz}. Such contour maps can become cluttered and often require a certain level of expertise to understand and gain insights from finer spatial resolution.

% While contour maps are adept at presenting 3D information in 2D space and providing a topographic view, they can become cluttered with limited data and often require a certain level of expertise to understand.
% Moreover, contour maps struggle to accurately represent feature relationships and to pinpoint events by their precise geolocation.
% For example, the National Climate Assessment (NCA) reports, published by the Intergovernmental Panel on Climate Change (IPCC), are projections derived from climate models \cite{reidmiller2017fourth}. 
% These reports offer direct forecasts of physical indicators for potential future climates, as well as indirect information about societal impacts. 
% Scientists leverage contour maps to visually interpret these downscaled climate projections. 
% However, traditional methods often rely on static contour depiction of high-resolution spatial data \cite{nayeem2022dcpviz}, leaving the useful underlying events and insights from finer spatial resolution.

In this context, user interactivity with contour maps has the potential to enhance the efficacy of such analyses. Furthermore, it is known that presenting more views (maps in this study) is beneficial for users in their sensemaking~\cite{andrews2010space, bradel2013large} and knowledge development~\cite{leigh2019usage} by providing a larger volume of information.  
For instance, they could assist users in identifying specific events or outlines and illustrating the relationships between their features based on user interactions. Nonetheless, quantifying these advantages in exploratory analyses presents a significant challenge. User interactions and visual representations could play a crucial role in organizing, structuring, and segmenting spatial data, facilitating user exploration from abstract overviews to focused inspections. 
They manifest in geospatial visualizations introduces new approaches to visual analysis, distinctively impacting human cognition.
% The way these interactions  manifest in geospatial visualizations introduces new approaches to visual analysis, distinctively impacting human cognition.

% Acknowledging these differences and the opportunities that they afford, visualization researchers have introduced a variety of interactive approaches to improve system usability and enhance cognitive engagement during the exploration of complex and large-scale datasets \cite{lu2017state}. The importance of user interactions in supporting exploratory geospatial analysis is widely recognized. Nevertheless, despite the qualitative evidence affirming their value, there is a lack of qualitative evaluations of these interactive features. Further research is necessary to comprehend and quantify the potential benefits offered by user interactions in geospatial visualizations designed for exploratory analytical tasks.

% Quantitative evaluation of the interactive visualizations generally involves a comparative user intervention study. A comparative study includes a reasonable number of participants investigating a set of items or performing analytical tasks with the comparative artifacts using selected datasets. The evaluation are formed by the metrics \cite{klavans2006quantitative} decided based on the dependent and independent variables in the study. There are several measures popularly taken to ensure the fairness and limit the bias in evaluation result. These measures includes same choice of dataset, balanced set of tasks for both artifacts, deciding fair measures of relatedness, recruiting participants with relevant expertise, and implement counter balancing for repeated measures \placeholder{\cite{}}.


% User interactions within visualization applications are often categorized according to the different analytical tasks they support \cite{afzal2019state}.


%To quantitatively evaluate interactive features in contour maps, both interactive and traditional static maps serve as comparative artifacts. To carry out such an evaluation, it is essential to define a series of exploratory tasks and the corresponding visual artifacts. Prior research has examined exploratory geospatial analysis from several perspectives, including event identification, comparison, ordering, and logical reasoning \cite{keller1994visual, koua2006, mayr2018integrated}. Furthermore, the choice of appropriate datasets, which contain sufficient information to reflect these analytical tasks, is crucial for the evaluation's outcome.

To evaluate the usability of interactivity in contour maps, we formulated the following research questions (RQs):
\begin{enumerate}[label=RQ\arabic*., leftmargin=* ]
    % \item \placeholder{HDY:todo}\rn{How does the accuracy and task completion time of participants using interactive contour maps compare to traditional static contour maps across various exploratory analysis task types?}
    \item What advantages in performance are expected when utilizing interactive contour maps in contrast to traditional static contour maps?
    
    % \item \HDY{What are the performance differences between using interactive contour maps and static contour maps for various exploratory analysis tasks?}

    % \item \placeholder{HDY:todo}\rn{What are the frequently used interactive features by participants when using interactive contour maps, how do these features contribute to their performance in different exploratory analysis tasks, and does user expertise play a role in this context?}  
    \item What interactive features are most useful or widely used for exploratory analysis tasks?
    % \placeholder{HDY:todo}\rn{What interactive features are most useful for exploratory analysis tasks?frequently used interactive features by participants when using interactive contour maps, how do these features contribute to their performance in different exploratory analysis tasks, and does user expertise play a role in this context?}  
\end{enumerate}
% \begin{itemize}[leftmargin=0.9cm]
%     \item [\textbf{RQ1}.] Do interactive features in contour maps enhance user task performance in terms of estimation accuracy and task completion time?
%     \item [\textbf{RQ2}.] Do interactive contour maps significantly outperform static maps in aiding users during various exploratory analysis tasks?
% \end{itemize}

% In this paper, we present the result of a crowd-sourced user intervention study aimed at quantitatively evaluating the role of interactive features in contour-based geospatial visualization that supports exploratory analytical tasks. 
% To address these RQs, we design and develop a web-based user interface that facilitates a user intervention study in an environment dedicated to exploratory contour map visualizations. A crowd-sourced user intervention
% study is conducted to examine the interactive features within the contour maps.
%This work presents the results of a crowd-sourced user study designed to quantitatively evaluate the role of interactive features in contour-based geospatial visualization for exploratory analytical tasks. 
% Drawing upon our literature review \cite{OGAO200223, koua2006} and collaboration efforts with the climate and environmental scientists \cite{nayeem2021visual, nayeem2022dcpviz, gdlviz2022}, we have selected seven exploratory visual analysis tasks to investigate the effectiveness of the interactive features in contour-based geospatial visualizations. 

To address these research questions, we conduct a crowd-sourced user study to evaluate the interactive features of contour maps. 
% A crowd-sourced user intervention study is then conducted to assess the interactive features within the contour maps.
% To answer these research questions, we create a web-based user interface for a dedicated environment focused on exploratory contour map visualizations. A crowd-sourced user intervention study is then conducted to assess the interactive features within the contour maps.
Drawing upon a literature review on previous research \cite{OGAO200223, koua2006,nayeem2021visual, nayeem2022dcpviz, gdlviz2022}, we select seven tasks and implement a web-based user interface utilizing two real-world geospatial datasets for the study. 
% The two datasets are temperature records for a tri-state area \cite{nytemperaturedata} and precipitation data for the contiguous U.S. (CONUS) \cite{Nemani2015}. 
% We employed two real-world geospatial datasets of different scales and features for the study, one comprising temperature records for a tri-state area \cite{nytemperaturedata} and the other featuring precipitation data for the contiguous U.S. (CONUS) \cite{Nemani2015}. 
% The data gathered from the user study are statistically analyzed to quantitatively understand the impact of user interactions on the execution of the specified exploratory analytical tasks.
% Data collected from the user study are statistically analyzed to examine the impact of user interactions on the execution of the specified exploratory analytical tasks.
Our findings suggest that the participants achieved greater accuracy using the interactive map compared to the static contour map, particularly in tasks such as associating, categorizing, clustering, identifying, and ranking the geospatial data points. 
% Section \ref{sec:task-specification} discuss the contextual definition of the participating tasks
Moreover, the results reveal that inspection and selection are the most frequently used interactive functions, followed by annotation, filter/search, and encode. These features are tailored to specific task types, such as annotations being mostly used in locate, rank, and associate tasks, while filter interactions are frequently utilized in identify and categorize tasks. The result also suggests that these features benefit the novice users, closing their performance gaps in complex exploratory tasks. 
% Our findings show that interactive contour maps enhance task accuracy compared to static visualizations. Notably, interactive features significantly improve task performance when identifying spatiotemporal differences within contours. We also provide a discussion on the participants' interaction behaviors and report a diagnostic analysis of their performance. 
These findings can be utilized as design considerations for crafting and assessing interactive contour maps designed for particular use cases related to exploratory geospatial analysis.

% THESE ARE FROM PAST SUBMISSIONS
% The insights collected serve as guidelines for designing and evaluating interactive contour maps tailored to specific use cases. 
% In this paper, we conduct a comparative user study to report a quantitative evaluation of the interactive features in geospatial visualization that supports exploratory analytical tasks. We leverage knowledge from the literature review to select seven exploratory visual analyses to investigate the usability of the interactive features in geospatial visualization. We illustrate geospatial data containing temperature records for the tri-state area \cite{nytemperaturedata} and precipitation data for the contiguous U.S. \cite{Nemani2015}. The collected data from the user study is statistically analyzed to understand the impact of the user interactions in performing exploratory analytical tasks. Our result shows that the interactive geospatial map improves the users' correctness of the performed tasks compared to the static geospatial visualization. Moreover, the interactive features significantly improve the performance of the users in identifying the spatiotemporal differences from the geospatial contours.

% This paper has the following contributions:

% \begin{enumerate}
   % \item We introduce a contour-based interactive geospatial visualization designed to support users in performing exploratory analytical tasks. Geospatial visualization consists of a wide range of features that allow users to inspect, select, annotate, and filter the geospatial data.
   % \item We designed a web-based user interface that facilitates a user intervention study in an environment dedicated to exploratory contour map visualizations. A crowd-sourced user intervention study was conducted to scrutinize the interactive features within the contour-based geospatial visualization.
   % \item We outline comprehensive guidelines for the visualization researchers to design analysis use-case-specific interactive visualizations for the contour-based geospatial data.
   % \item We provide a discussion on the participants' interaction behaviors and report a diagnostic analysis of their performance. The insights collected serve as guidelines for designing and evaluating interactive geovisualizations tailored to specific use cases. 
% \end{enumerate}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/map-view.png}
    \caption{
    Illustration of two interactive contour-based geospatial visualizations:  (A) temperature intensity in New York City and (B) precipitation intensity in the contiguous U.S. recorded at a certain time. 
    % Illustration of two interactive contour-based geospatial visualizations presenting (A) temperature intensity in New York City and (B) precipitation intensity in the contiguous U.S. recorded at a certain time. 
    % The interactive features in the map are intended to support exploratory visual analysis providing underlying information about the contour regions.
    % The interactive features in the map are intended to support exploratory visual analysis of the contour regions.
    The interactive features are intended to support exploratory visual analysis of the contour regions.
    }
    \label{fig:map-view}
\end{figure*}


==> sections/Prev/2-related-works.tex <==
\section{Related Works}
% In this section, we summarize the previous research in visualizing the geospatial data that enables users to conduct exploratory visual analyses. In addition, we review the methods and techniques in evaluating the usability of the geovisual environments.

\subsection{Geospatial Visualization}
% Geospatial data are traditionally categorized into three types: raster data, vector data, and network data \cite{alam2021survey, LEE201574}. Raster data comprise an extensive array of pixels, each representing a specific geographic location. This type of data often illustrates both discrete information (e.g., terrain types) and continuous information (e.g., temperature or land elevation). In contrast, vector data contains information such as the location of specific points of interest (e.g., a movie theater), the path of linear structure (e.g., roads or rivers), and the area of spatial entities (e.g., countries, rivers, or national parks)\cite{alam2021survey}. This data is often represented by points, lines, or polygons. The third type, network or graph data, illustrates the spatial connectivity among the nodes in the vector data such as road transportation routes and navigation systems \cite{andrienko2007geo, huang2009supporting}. In addition to these spatial features, dimension-impacting factors like time are frequently associated with the geospatial data \cite{pelekis2004literature, shekhar2015spatiotemporal}.

Visualization researchers have introduced many geovisual environments for various data types, analysis requirements, and use cases. The potential of geospatial data through geographic information systems for mapping and analytics has been realized beyond domains related directly to earth science. Such domains, including traffic systems, energy systems, health informatics, and entertainment, heavily rely on the location or geographical data \cite{poweroflocation}. Choropleth, point map, cluster map, cartogram maps, etc. are popularly employed to visualize the data with spatial dimensions \cite{Maskey2020, Tominski2021, nayeem2022dcpviz} depending on analytic necessity. 
% While choropleth and cluster maps are popular for displaying spatial categorical information \cite{gdlviz2022},
While choropleth maps are a common way to display discrete interval or ratio scaled data \cite{gdlviz2022}, heatmap and distribution maps often illustrate continuous data variables containing geo-coordinated attributes  \cite{Quinan2016}. Despite this variety, to the best of our knowledge, we have 
 yet to encounter any interactive contour map specifically designed to provide an exploratory geovisual environment for spatial data analysis.
 % **plot the idea of interactive contour supporting the use cases for various analytic needs.

Traditionally, users often rely on static geospatial depictions where information is visually estimated from traditional geospatial views, typically in the form of raster images. Notable examples of tools facilitating this approach include NASA's Panoply software package, which extracts high-dimensional climate datasets from memory efficient encodings and visualize them as geospatial contours \cite{2018AGUFMIN21B35A}, and  QGIS \cite{Hugentobler2008}, a widely used open-source cross-platform software that visualizes geospatial data in various format (e.g., GeoJSON, NetCDF, Shapefile) as a mesh layer. In addition, toolkits such as MATLAB \cite{hanselman1996mastering}, NCAR \cite{NCAR2019}, and GrADS \cite{Berman2001} remain popular for visualizing geospatial data. The Geospatial contours generated by these toolkits are frequently used by domain researchers to illustrate the results of their analyses \cite{gibson2017use, CAO2021145320}. However, these traditional approaches are often static, limiting the scope and depth of data interaction and exploration.

Moreover, we have examined the transformations of geospatial visualizations to accommodate multi-dimensional attributes. For instance, Community Data Analysis Tools (CDAT) provide a software infrastructure and platform for analyzing multidimensional data \cite{williams2002climate, potter2009visualization}, which is widely used for distributed analyses of geospatial data. In addition, CDAT offers a visualization and control system that interacts with Python to visualize geospatial data \cite{williams2002climate}. GIS4WRF \cite{MEYER2019166} is another toolkit for processing and visualizing weather data and forecasting NetCDF in an interactive single graphical environment. MeteoInfo is a desktop application that provides a geospatial visualization platform for multidimensional meteorological data \cite{wang2014}. Moreover, ClimateData.US provides an interactive geovisual interface that provides comparative visualization of climate data in different emission scenarios \cite{Herring2017}. Geospatial views are developed for visualizing time-varying data and performing rule-based associations \cite{wang2018}. However, these visualization approaches often lack adequate interactive features for the diversified exploration of spatial data variables.

\subsection{Evaluating Geovisual Environments}
% Evaluations of geovisual environments include various qualitative and quantitative measures. Tools and applications employed for geospatial visual analysis are often tailored to specific use cases. 
% Therefore, qualitatively evaluating the usability of those tools is mostly sufficient with the domain experts' or corresponding users' feedback \cite{Sanyal2010, nayeem2022dcpviz}. 

The evaluation criteria of geovisual environments range from the ability to display the data, the interactivity for analytical tasks, and the self-explanatory attributes of the visualizations \cite{johansson2010evaluating}. It generally involves visualization researchers developing geovisual components followed by user experts interacting with it and providing constructive feedback for the next iteration or outlining the usability for intended analysis purposes \cite{nayeem2021visual, nayeem2022dcpviz, gdlviz2022}. 
For example, Koua et al. \cite{koua2006} conducted a user study with geographers, cartographers, geologists, and environmental scientists and evaluated the usability of different visualization methods for geovisual analyses. 
% Koua et al. \cite{koua2006} conducted a user study with geographers, cartographers, geologists, and environmental scientists as participants where they evaluated the usability of different visualization methods for geovisual analyses. 
Their study included visualization such as parallel coordinates, and self-organizing heatmap representation against the geospatial map to evaluate users' performance in 10 exploratory analytical tasks such as categorizing, clustering, and identifying spatial areas. 
% Robinson et al. \cite{robinson2017} conducted a user study to evaluate, STempo, a geovisual environment consists of coordinated multiple view (CMV), desgined for exploring spatial, temporal, and categorical aspect of hierarchical event data.  
% Robinson et al. \cite{robinson2017} conducted a user study to evaluate, STempo, a geovisual environment consists of coordinated multiple view (CMV), desgined for exploring spatial, temporal, and categorical aspect of hierarchical event data.  
% Zahan et al. \cite{zahan2021contour} compared four design techniques for contour line stylization to visualize the multivariate geospatial data. 
% While stylization presents the multivariate associations in a unified view, other potentials of contour maps such as categorizing, clustering, and identifying spatial areas are still to be explored. 


% In our review, we only found a handful of literature that quantitatively evaluated geovisual environments with users from a diverse range of expertise and the effect on their performance.
In our review, we found a small amount of literature that quantitatively evaluated the interactivity of geovisual environments with users from a diverse range of expertise and the effect on their performance.
Nagel et al. \cite{nagel2012} introduced a tabletop map visualization that enables users to explore geospatial networks interactively. Mahmood et al. \cite{mahmood2019improving} presented a mixed reality geospatial visualization method that fosters remote collaboration and knowledge sharing for sensemaking tasks. Herman et al.~\cite{herman2018evaluation} evaluated the interactivity of 3D maps for tasks such as landscape management, and crisis management. They suggested that interactive 3D maps are better suited for complex tasks, allowing users to make more accurate decisions in less time. 
Amini et al.~\cite{amini2014impact} pointed out that 2D maps have limitations in visualizing movement data, such as car and plane trajectories when trajectories overlap. They investigated the effect of interactive 2D and 3D maps on analyzing movement data and reported that participants performed better with the 3D map than with the 2D map. \HDY{Lateh and Raman~\cite{lateh2005study}} examined the static and interactive 2D maps in learning and teaching geography in a high school. They found that the interactive map significantly enhances the students' ability to read and understand spatial information on the map. However, earlier studies investigated the effect of map interactivity on limited tasks such as value identification and finding clusters. 

Roth \cite{roth2013empirically} developed a functional taxonomy of interaction for cartography and geospatial visualizations. The preemptive definitions from the study were separated into interaction objectives and operators, which serve as a structure to study user interactions for map-based visualizations. The foundational knowledge for designing cartographic view outlined in Roth \cite{roth2013empirically} and the exploratory geospatial task classification presented by Koua et al. \cite{koua2006} are relevant to the scope of this study design for quantitative evaluation.


==> sections/Prev/3-interactive-visualization.tex <==

\section{Contour-based Geovisualization}

% \HDY{In this section, we define terms and describe specific tasks and interactive features for contour-based geovisualization. }
This section defines terms and describes specific tasks and interactive features for contour-based geovisualization. 

\subsection{Interactive and Static Contour Map}
The geospatial map is a multi-layered view comprising a base map, contour map, and spatial masks. 
% In the realm of Geographic Information Systems (GIS), 
The base map signifies a collection of geographic features that illustrate the background scene for a given location. 
% We utilize OpenStreetMap \cite{openstreetmap} as our base map to show geographical features such as boundaries, rivers, and highways. % for the user's area of interest. 
The contour map provides a topographic representation of a location, clustering areas of identical value with lines and polygons \cite{hahmann2015contour}.  Next, the spatial masks outline boundaries for the contiguous US regions providing a visual segmentation of area-specific (regional) intensity. 


% Despite this multi-layered version of the geospatial contour map offering the capacity to accommodate interactive features beyond a traditional single-layer bitmap, we categorize this map as a static one within our user study.



Within the contour layer, boundaries create multiple polygons that we identify as contour regions. For example, the contour maps in Fig. \ref{fig:map-view}A and B illustrate the temperature intensity for New York City, and the precipitation intensity for the contiguous US respectively. On one hand, we define an interactive contour map as a map that has the capability to include interactive features. 
% An interactive contour map, for example, could have the capability to calculate the total number/area of regions corresponding to unique intensity values. 
An interactive contour map, for example, could have the capability to present the total area of regions corresponding to unique intensity values. 
% In order to calculate the contour area distribution, we classify the contour map according to areas that share equal value or intensity range. 
% Subsequently, we compute the area sum for all the contour regions grouped by unique value or intensity range. 
This allows the user to measure the intensity distribution or spread within the area of interest based on values of interest. 
On the other hand, we \HDY{define} a static contour map as a map which does not offer the capacity to accommodate interactive features beyond the traditional approach.

% Despite this multi-layered version of the geospatial contour map offering the capacity to accommodate interactive features beyond a traditional single-layer bitmap, we categorize this map as a static one within our user study.

\subsection{Visual Exploratory Tasks}\label{sec:visual-tasks}

We review a set of exploratory analysis tasks previously used in evaluating exploratory geovisual environments \cite{keller1994visual, koua2006}. 
This study utilizes the exhaustive list proposed by Keller et al. \cite{keller1994visual} and subsequently employed by Koua et al. \cite{koua2006} for a usability study in contour-based exploratory geovisualization. The identified tasks are low-level analytical tasks which are common among climate and environmental scientists \cite{koua2006, nayeem2022dcpviz, zahan2021contour, gdlviz2022}. 
 % derived from the selected exploratory task types are
Although these tasks are applicable to various types of map visualizations, we selected the following seven tasks because they are suitable for the contour map based on their operations:


\begin{enumerate}[leftmargin=* ]
    \item \textit{\textbf{Associate}} tasks involve users in finding similarities between data points based on the characteristics of attributes, geographic locations, and patterns of events.

    \item \textit{\textbf{Categorize}} tasks require defining all regions on the display by the boundaries. The regions are usually categorized by common features or spatial positioning.

    \item \textit{\textbf{Cluster}}-type tasks require users to identify different groups of similar data points or regions within the geospatial data. 
    % In these tasks, the user identifies sparse data points or regions that share common attributes to form unique groups within the data.

    \item \textit{\textbf{Distinguish}} analytical tasks require users to identify the differences or variations in geospatial areas or locations.
    % two contours . These differences often include the geospatial area or location and values of the same attribute.

    \item \textit{\textbf{Identify}} demands establishing the relationship between data attributes based on their shared characteristics.

    \item \textit{\textbf{Locate}} is identifying certain range of data points or events on the map. 
    % In this task, we aim to evaluate whether the map supports the user in locating the facts or a range of values.

    \item \textit{\textbf{Rank}}-type tasks require feature ordering based on data attributes, clusters, or geographic locations.
\end{enumerate}

% \subsection{Contour Area Distribution}
\subsection{Interactive Features} \label{sec:user-interactions}

% The user interactions facilitate human cognition processing and are categorized based on their capabilities to support exploratory analysis within geospatial data \cite{lu2017state}.
% The user interactions facilitate human cognition processing and are designed to support the exploratory analysis task \cite{lu2017state}.
The user interactions are designed to support the exploratory analysis task by facilitating human cognition processing \cite{lu2017state}.
% discussed later in Section \ref{sec:task-specification}. 
% To find these interactive features, we have gathered insights from our previous research \cite{nayeem2022dcpviz, gdlviz2022, nayeem2021visual} as well as our literature review \cite{wang2018, Herring2017, McLean2020}. 
To find these interactive features, we have gathered insights from literature review \cite{nayeem2022dcpviz, gdlviz2022, nayeem2021visual, wang2018, Herring2017, McLean2020}. 
% Roth \cite{roth2013empirically} defined what interaction means, its purpose, criteria for relevant applications, and fundamental interaction design in the context of cartography. 
For example, DiBiase's Swoopy schematic \cite{dibiase1990visualization} provided a framework, that includes exploration, analysis, synthesis, and presentation, to identify the purpose of maps. 
% Therefore, it is leveraged to hypothesize the potential of interactions in the exploratory geovisual environments. 
% The following interactive features are identified.
Based on previous research, we identified a set of interactive features including \textit{\textbf{Inspection, Selection, Annotation, Filter, Encoding,}} and \textit{\textbf{Synchronization}}. In the following section, we discuss them in detail along with our implementation.

Please note that interactive maps usually provide navigational features like zooming and panning. However, we do not include them in this work because our major concern is to investigate the usability of user interactions with contour regions. 
% However, these interactions are not included in our features beacuase our focus is primarily on the usability of the user interactions with the contour regions. 


==> sections/Prev/4-hypotheses.tex <==
\section{Web Interface for user study }

% mention leaflet and concisely desribe our contribution in implementing interactive features
For our user study, we designed and developed a web interface that includes multiple coordinated visual and interactive components (Fig. \ref{fig:interaction-teaser}) \footnote{ \url{https://vizus.cs.usu.edu/app/geospatial-study}}. 
% \footnote{ \url{https://geospatial-study.vercel.app/training}}. 
%For the user intervention study, we designed a web-based interactive interface.%  
% The user study interface is developed on React.js using D3.js and Leaflet.js for interactive visualizations, Django for the API server, and MongoDB for storing the application and user data. 
The interface is built with React.js and incorporates D3.js and Leaflet.js for interactive visualizations. It utilizes OpenStreetMap (OSM) \cite{openstreetmap} as its base map to show geographical features such as boundaries, rivers, and highways. It is worth noting that OSM employs the Web Mercator projection, which can introduce considerable distortions in regions near the poles, potentially complicating area comparisons.  However, since our maps are primarily focused on regions within the US, the impact of this limitation is substantially reduced. Django and MongoDB are utilized for the API server and database to store user interaction logs. 
% It uses Django for the API server and MongoDB to store both application and user data. 
% These components are 1) a geospatial map, 2) a contour area distribution view, and 3) interactive features including inspection, selection, exploration, toggle layers, draw markers, control visibility, and location search.

% The visual components illustrate the geospatial information with or without interactive features described in Section~\ref{sec:user-interactions}.
% The visual components illustrate the geospatial data (commonly in the GeoJSON format) and basic mapping to the geographic location without leveraging the interactive features. 
% For visualizing the transformed geospatial contour into GeoJSON, we utilized the Leaflet.js library. 


\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/geospatial-study-teaser-dy.png}
  \caption{
    Overview of the quantitative evaluation for contour-based interactive geospatial visualization: We conducted a crowd-sourced study to measure user performance in exploratory analysis tasks. We compared (A) a traditional static contour map with (B) a contour-based interactive geospatial visualization. The results (C) suggest that interactive features significantly improve performance in complex tasks such as spatial data association, categorization, clustering, and ranking.
  }
  \label{fig:interaction-teaser}
\end{figure}


\subsection{Geospatial Datasets}
% In this study, we examine contour-based geospatial visualizations under two distinct scenarios: 
Two separate geospatial datasets are employed to visualize contour maps for distinct scenarios:

% For this purpose, we employ real-world geospatial data sourced from two distinct origins:
%In this study, we scrutinize the contour-based geospatial visualization under two scenarios, presenting the long and short extent of the geospatial data. Hence, we observe whether the geographical extent and data granularity has an impact on the quantitative evaluation of the interactive features. We present geospatial visualization utilizing the data generated from two different sources: 

\begin{itemize}[leftmargin=* ]
    \item \textit{\textbf{NY Temperature:}} Hourly-averaged temperature forecast for the tri-state area (Fig. \ref{fig:map-view}A) based on the Weather and Research Forecasting (WRF) model published by Coastal Urban Environmental Research Group (CUREG) \cite{nytemperaturedata}
    % it provides temperature data (D\textsubscript{T}) for a limited spatial extent around New York.
    
    \item \textit{\textbf{CONUS Precipitation:}} Monthly-averaged precipitation projections for the CONUS published by NASA Earth eXchange (NEX) where downscaled climate projections (NEX-DCP30) are generated in different emission scenarios such as RCP 2.8, RCP 3.5 and RCP 4.5 \cite{Nemani2015}, as shown in Fig. \ref{fig:map-view}B
    % it provides precipitation data (D\textsubscript{P}) for the contiguous U.S., covering a larger area than \textit{NY Temperature}.
\end{itemize}
 
% Maps can either be a single contour or two contours provided side-by-side for comparative analysis. We use two different types of data.


\subsection{Interactive Geospatial Map and Interactions}
The interface displays one or two contour-based geospatial maps based on a study condition discussed in Section~\ref{section_map_layout}. When multiple maps are provided, they are uniformly either static or interactive. 
When a contour-based map is interactable, it supports the interactions identified in Section~\ref{sec:user-interactions}. Please note that \HDY{the} \textit{\textbf{Synchronization}} feature is always supported when two interactive maps are presented in the interface.
The following demonstrates our implementation for the interactive features.
% , shown in Fig. \ref{fig:interaction-teaser}-d.

% An implementation of the contour-based interactive geospatial map shown in Fig. \ref{fig:map-view}, demonstrates the interactive features selected for this user study. 

\begin{itemize}[leftmargin=* ]
\item \textit{\textbf{Inspection}} allows the user to investigate a contour region. When the user hovers the pointer over the region, it highlights all the associated contour regions on the map and shows a tooltip. 
% This interaction allows the user to hover the mouse cursor over a contour region, which then highlights all the associated contour regions on the map. 
The tooltip provides additional information about the interacted region, the number of contour regions occupied by that intensity, and the contour area distribution for those regions.

% \item \textbf{Selection:} Upon each selection or deselection of a region on the map by click, the contour area and regions are recalculated based on the updated selection. \rn{Selecting a point on the map places a marker that provides details about the intensity, occupied cluster area, and comparing measures.}
\item \textbf{Selection} or deselection of a region of interest is accomplished by clicking the mouse on the map or one of the contour labels (Fig. \ref{fig:map-view}F). The region of interest can be either a contour region or a location on the map.
% It places a marker that provides details about the intensity, occupied cluster area, and comparing measures. 
% It places a marker displaying details such as intensity, occupied cluster area, and comparative measures. 
Following the selection, the contour area and regions are recalculated to reflect the updated selection.
% Upon each selection or deselection of a region on the map by click, the contour area and regions are recalculated based on the updated selection. 
% \rn{Selecting a region of interest on the map places a marker that provides details about the intensity, occupied cluster area, and comparing measures.}

\item \textit{\textbf{Annotation}} places a marker displaying details such as intensity, occupied cluster area, and comparative measures. 
% enables the user to place markers on the map. 
A right mouse click on a point of interest enables the user to place a marker on the map, as depicted in Fig. \ref{fig:map-view}C. 
The view allows multiple markers across different locations. When a user clicks one of the markers with the mouse's left button, it displays contour information for that marker as well as other markers to aid in comparison. 

% \item \textit{\textbf{Annotation}} enables the user to place markers on the map. 
% A right mouse click on a point of interest places a marker on the map, as depicted in Fig. \ref{fig:map-view}C. 
% The view allows multiple markers across different locations. When a user clicks one of the markers with the mouse's left button, it displays contour information for that marker as well as other markers to aid in comparison. 


\item \textit{\textbf{Filter/Search}} aids the user in locating specific areas or boundaries on the map that might otherwise be difficult to find manually. 
The interactive map features a search icon positioned at its top right corner, as illustrated in Fig. \ref{fig:map-view}E. The user can type the name of the desired area, and select the appropriate option from the provided list. 
% To initiate a search, the user can click on the search icon placed at the top right of the contour map (Fig. \ref{fig:map-view}E), type the name of the desired area, and select the appropriate option from the provided list. 
A marker will then be placed on the chosen location. 
% These markers generated through the search function operate in the same manner as the other annotation markers placed on the map.
The marker operates in the same manner as annotation markers.


% \item \textit{\textbf{Filter/Search}} \HDY{todo} provides search capabilities within the contour. 
% The search function aids the user in locating specific areas or boundaries on the map that might otherwise be difficult to find manually. 
% To initiate a search, the user can click on the search icon placed at the top right of the contour map (Fig. \ref{fig:map-view}E), type the name of the desired area, and select the appropriate option from the provided list. 
% % A marker will then be placed on the chosen location. These markers generated through the search function operate in the same manner as the other annotation markers placed on the map.
% These markers generated through the search function operate in the same manner as annotation markers.

\item \textit{\textbf{Encoding}} enables the user to control the visibility of the contour area or border. The interactive map provides three sliders to control fill opacity, border opacity, and border strength as shown in Fig. \ref{fig:map-view}D.
% Contour styles allow for manipulation of the transparency or strength of the contour area and border. 
This improves the user's ability to better correlate an event with its geographical location, as well as, allows the user to change the visual configuration to perceive insights from a cluttered view.

% \item \textit{\textbf{Encoding}} \HDY{todo} enables the user to control the visibility of the contour on the geographical boundary. 
% Contour styles allow for manipulation of the transparency or strength of the contour area and border. 
% This improves the user's ability to better correlate an event with its geographical location, as well as, allows the user to change the visual configuration to perceive insights from a cluttered view.


\item \textit{\textbf{Synchronization}} makes it easier to compare two contour maps, allowing for exploratory analysis of potential differences at points of interest. In this configuration, all previously discussed interactions are synchronized, which means that any user interaction with one contour map has a complementary effect on another. 

% \item \textit{\textbf{Synchronization}} facilitates comparisons between two contour maps, providing exploratory capabilities to identify potential differences at points of interest. 
% In this setup, all previously discussed interactions are synchronized, meaning any user interaction with one contour map has a complementary effect on the comparative map. 
% % This study presents these comparative maps as `Snapshot Left/Right.'
\end{itemize}

% \subsection{\placeholder{how can participants answer the questions?}}
% \placeholder{need Raihan's input}

% \paragraph{\textbf{Inspection:}} 
% This interaction allows the user to investigate a contour region. When the user hovers the mouse over the region, it highlights all the associated contour regions on the map and shows a tooltip. 
% % This interaction allows the user to hover the mouse cursor over a contour region, which then highlights all the associated contour regions on the map. 
% The tooltip provides additional information about the interacted region, the number of contour regions occupied by that intensity, and the contour area distribution for those regions.
% % In addition. a tooltip pops up, providing additional information about the interacted region, the number of contour regions occupied by that intensity, and the contour area distribution for those regions.

% \paragraph{\textbf{Selection:}} 
% % This interaction allows the user to enable or disable all the contour regions of a particular intensity. 
% The user can select a region of interest by clicking the contour labels (Fig. \ref{fig:map-view}F). 
% % The user can click on the contour labels (as shown in Fig. \ref{fig:map-view}F) to select the events of interest. 
% Upon each selection or deselection, the contour area and regions are recalculated based on the updated selection. 

% \paragraph{\textbf{Annotation:}} 
% % We incorporated an annotation feature enabling the user to place markers on the map for detailed exploration or comparison with other locations or regions. 
% This feature enables the user to place markers on the map. 
% A right mouse click on a point of interest places a marker on the map, as depicted in Fig. \ref{fig:map-view}C. 
% The view allows multiple markers across different locations. 
% % A left click shows additional information, essentially performing an inspection of the marked location and comparing it with the other marked places.
% When a user clicks one of the markers with the mouse's left button, it displays contour information for that marker as well as other markers to aid in comparison. 


% \paragraph{\textbf{Filter/Search:}} 
% This interaction provides search capabilities within the contour. 
% The search function aids the user in locating specific areas or boundaries on the map that might otherwise be difficult to find manually. 
% To initiate a search, the user can click on the search icon placed at the top right of the contour map (Fig. \ref{fig:map-view}E), type the name of the desired area, and select the appropriate option from the provided list. 
% % A marker will then be placed on the chosen location. These markers generated through the search function operate in the same manner as the other annotation markers placed on the map.
% These markers generated through the search function operate in the same manner as annotation markers.

% \paragraph{\textbf{Encode:}} This interaction enables the user to control the visibility of the contour on the geographical boundary. Contour styles allow for manipulation of the transparency or strength of the contour area and border, enhancing the user's ability to better correlate an event with its geographical location.

% \paragraph{\textbf{Synchronize:}} This facilitates comparisons between two contours, providing exploratory capabilities to identify potential differences at points of interest. 
% In this setup, all previously discussed interactions are synchronized, meaning any user interaction with one contour map has a complementary effect on the comparative map. This study presents these comparative maps as `Snapshot Left/Right.'
% %and `Snapshot Right'.


% In in Fig. \ref{fig:map-view}E, the bar chart presents these categorical data that allows user to perceive the range of intensities are prominent or faint on the contour map.

% The interactive map also provides basic navigation interaction such as zooming and viewport dragging.
% Interactive maps usually provide navigation features including zooming and panning. 
% However, these interactions are not included in our analysis as our focus is primarily on the usability of the user interactions with the contour regions. 
% In this work, however, these navigation features are not included as our focus is primarily on the usability of the user interactions with the contour regions. 



% The features included were chosen based on their potential to support exploratory analysis tasks discussed later in Section \ref{sec:task-specification}. 
% That entails there is considerable scope for incorporating additional interactive features that may be suitable for specific cases. 


% \subsection{Geospatial Map}
% The geospatial map is a multi-layered view comprising a base map, contour map, and spatial masks. In the realm of Geographic Information Systems (GIS), the base map signifies a collection of geographic features that illustrate the background scene for a given location. 
% We utilize OpenStreetMap \cite{openstreetmap} as our base map to show geographical features such as boundaries, rivers, and highways. % for the user's area of interest. 


==> sections/Prev/5-task-specification.tex <==
\section {Crowd-sourced user study}
% \placeholder{Request from DY: There is no explanation about map layout (\textit{single vs. multi map}) and geospatial expertise (\textit{novice vs. experienced}) + interaction logs . Please add them in this section. }


Our study design is influenced by a literature review on crowd-sourced studies evaluating visualization components \cite{heer2010, nagel2012, karduni2021} that provided a well-grounded idea on participant recruitment and exclusion criteria, training requirements and study procedures. 




\subsection{Participants \& Recruitment}
\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}

    \includegraphics[width=0.9\linewidth]{figures/demographic-summary.png}
    \caption{Summary of 62 participants' educational qualifications, computer usage, geospatial expertise, and visualization expertise. }
    \label{fig:demographic-data}
\end{figure}
We host the study online, with participants sourced from Amazon Mechanical Turk (MTurk). Our user study interface is directly linked to a Human Intelligent Task (HIT) we posted on the MTurk portal. % that links to our user study interface. 
To ensure the quality %cleanliness
of the collected data, we selected participants from MTurk who had an approval rating above 95\% and were identified as master workers. In line with our pre-registration criteria, we exclude participants who failed engagement questions or completed the study in under 8 minutes. This led to a final sample size of 62 participants (25 females and 37 males). 
% Our a-priori power analysis using the G* power application \cite{faul2009statistical} indicates that our sample size of 62 estimated achieves power over 0.994. 
We ask the participants about their academic qualifications, their daily computer usage, and how they rate their expertise in perceiving visualization and analyzing geospatial data. 
For computer usage, visualization expertise, and geospatial analysis expertise, the participants identify themselves from the groups shown in Fig. \ref{fig:demographic-data}. 
% We found that 80\% participants have at least a bachelor's degree and all of them use computers for their daily tasks. 
They identified themselves as having various levels of expertise in visualization and geospatial analysis (Fig. \ref{fig:demographic-data}). 
% Each participant earned a \$4 incentive for their effort and contribution to our user study.
Each participant earned a \$4 incentive for their contribution to our user study.
On average, they took 8.6 minutes (\textit{SD=7.99}) for the training session and 29.14 minutes (\textit{SD=19.75}) to complete the main session.




==> sections/Prev/6-user-study.tex <==
% \section{User Study}
% \ic{removed Figure 1, and let's use figure 2 as a teaser}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/map-view.png}
%     \caption{Illustration of two interactive contour-based geospatial visualizations presenting (A) temperature intensity in New York City and (B) precipitation intensity in the contiguous U.S. recorded at a certain time. The interactive features in the map are intended to support exploratory visual analysis providing underlying information about the contour regions.}
%     \label{fig:map-view}
% \end{figure*}

% We provided analytical tasks for eight single-map/multi-map scenarios. As we are using two different datasets (temperature and precipitation), it offered us to evaluate various interactive features. Hence, we leveraged the format specified in Section \ref{sec:task-specification} to create variants of analytical tasks for each type.


\subsection{Study Factors}

\subsubsection{Map Type}
% \HDY{static map vs. interactive map}

In this work, we divide map types into two categories: static map (Fig. \ref{fig:interaction-teaser}A) and interactive map (Fig. \ref{fig:interaction-teaser}B), based on their level of interactivity. The interactive map supports the aforementioned interactive features. 
Please keep in mind that the interactive map provides all the features, and we do not exclude or omit any specific features.  We made this decision to ascertain and discuss which interactive features participants commonly utilize to accomplish the tasks. Conversely, the static map is designed considering the traditional approach of contour maps and only offers panning and zooming capabilities.

% We identify the participating map types as the traditional static contour map (Fig. \ref{fig:interaction-teaser}A) and interactive contour-based geospatial visualization (Fig. \ref{fig:interaction-teaser}B).

\subsubsection{Map Layout}\label{section_map_layout}
% \HDY{single map vs. multi map ...}
The map layout includes two conditions: single map and multiple map. The single map condition provides only one static or interactive map, as the name implies. The multiple map displays two maps side by side, with each map potentially containing data from different locations or time periods. We refer to them as Snapshot Left/Right. They are either static or interactive maps.


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\bgroup
\def\arraystretch{1.2}%
\begin{table*}[h]
\centering
\caption{The participants performed these exploratory geovisual analyses from seven unique task types. These exploratory tasks are designed for both single and multiple map layouts to evaluate the usability of interactive features in a geovisual environment.
}
\begin{tabular}{| p {5em}| p {24em} | p{25em} |}
\hline
\textbf{Task Type} & \textbf{Single Map}                                                                                                                                                                                          & \textbf{Multiple Map}                                                                                                                                                                            \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Associate          & Based on the area covered which two \emph{[variable/marker]} intensities below are the most similar?                                                                                    & Find the \emph{[variable/marker]} intensities from both snapshot that cover the \emph{[largest/smallest]} area.                                        \\ \hline
Categorize         & What is the \emph{[area/intensity]} (difference) for the \emph{[highest intensity/largest area]} recorded on \emph{[contour/Location X]}? & What is the area difference of \emph{[variable]} \emph{[intensity]} between Snapshot Left and Right?                                                   \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Cluster            & How many \emph{[unique/total]} contour regions are visible on the map?                                                                                                                  & How has the number of \emph{[unique/total]} contour regions changed from `Snapshot Left' to `Snapshot Right'?                                                               \\ \hline
Distinguish        & What is the \emph{[area/intensity]} difference between the highest and lowest \emph{[variable]}?                                                                   & How does the \emph{[highest/lowest]} intensity shift from `Snapshot Left' to `Snapshot Right'?                                                                              \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Identify           & What is the \emph{[intensity/difference between]} \emph{[variable]} in Location \emph{[X]} (and Location \emph{[Y]})?    & What is the intensity difference between Location \emph{[X]} in `Snapshot Left' and Location \emph{[Y]} in `Snapshot Right'?                           \\ \hline
Locate             & What is the \emph{[highest/lowest]} intensity on the \emph{[contour/marked area]}?                                                                                 & What is the \emph{[highest/lowest]} intensity \emph{[between both snapshots/among all markers]}?                                                       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
Rank               & Order the \emph{[markers/intensities below]} from \emph{[high to low/low to high]} \emph{[intensity/area]}.                                   & Order the snapshots based on the \emph{[larger/smaller]} area covered by the \emph{[lowest/highest]} \emph{[variable]} intensity. \\ \hline
\end{tabular}
\label{tab:exploratory-tasks}
\vspace{-.3cm}
\end{table*}


\subsubsection{Exploratory Tasks}
In this work, we consider the seven visual exploratory tasks identified in Section~\ref{sec:visual-tasks}. These exploratory tasks can be categorized based on the number of data points they encompass. These tasks are broadly grouped into simple and complex tasks. Simple tasks involve a more direct spatial exploration, primarily focusing on  \textit{distinguish}, \textit{identify}, and \textit{locate} task types. Here, users typically interact with no more than two data points. The essence of these tasks is to either determine the location of a known event or ascertain the event based on its location. 
% and querying the location of where it happened or vice-versa. 
In contrast, complex tasks delve into a deeper spatial analysis, encapsulating \textit{associate}, \textit{categorize}, \textit{cluster}, and \textit{rank} tasks. %type of spatial analysis where the user explore the relationships among multiple data points. 
Here, the exploration revolves around discerning between numerous data points. Users predominantly seek data similarities, often independent of specific locations or events.

For the design of these tasks, we consider both singular and comparative explorations of geospatial data. The synchronized interactions within the map are tailored to aid users in juxtaposing events across multiple maps, a technique prevalent in temporal-spatial data research. While a singular map is adept at providing insights into a specific geospatial event, our aim is to discern the advantages interactive features confer when analyzing spatiotemporal discrepancies. Consequently, our task designs cater to both individual and multi-map analytical explorations. The comprehensive list of these tasks is presented in Table \ref{tab:exploratory-tasks}. Please refer to the supplementary materials for a complete list of questions.
While we acknowledge that the analytical tasks in Table \ref{tab:exploratory-tasks} may span multiple types, we have designated each based on its most dominant analytical characteristic. These tasks involve multiple-choice questions, where participants select one correct answer from three options. % We opted to offer fewer options to simplify our task, considering that not all participants may be acquainted with visual analytics.}

\subsubsection{Others}
% \paragraph*{Map Data Context}
\hspace{\parindent}\textbf{Map Data Context:}
To examine the general effect of interactive features, two datasets with different spatial ranges are utilized in this study (i.e., NY Temperature and CONUS Precipitation).
On one hand, NY Temperature provides temperature data (D\textsubscript{T}) for a limited spatial extent around New York. 
On the other hand, CONUS Precipitation provides precipitation data (D\textsubscript{P}) for the contiguous U.S., covering a larger area than \textit{NY Temperature}.
% The numbers following D\textsubscript{T} and D\textsubscript{P} in Table~\ref{tab:task-distribution} refer to unique instance of the data.
The numbers following D\textsubscript{T} and D\textsubscript{P} in Table~\ref{tab:task-distribution} refer to the distinct subsets of data. The seven questions for the multi map task sets in Table \ref{tab:exploratory-tasks} are developed using the two datasets separately. 
 


% \placeholder{ The temperature data (D\textsubscript{T}) for New York City spans a limited spatial extent, allowing the exploration of interactive features such as inspection, search, marking, encoding, and synchronized interaction.}

% \placeholder{On the other hand, the precipitation data (D\textsubscript{P}) for the CONUS covers a broader area, offering the opportunity to experiment with additional interactive features such as region/state selection, data filtering, and viewport shifting. To complement the repetitive measurements outlined in Table \ref{tab:task-distribution}, we include six distinct instances of temperature and precipitation data, each recorded at different times.}

\textbf{Participants' Expertise:} We consider the participants into two groups - novice and experienced, based on their reported expertise in geospatial analysis. 
The participants who identified themselves as \textit{`unfamiliar'} or \textit{`somewhat familiar'} with geospatial analysis are classified as novice users, and the other participants who identified themselves as \textit{`somewhat experienced'}, \textit{`experienced'}, or \textit{`expert'} are classified as experienced users. 
% In contrast, participants who identified themselves as \textit{`somewhat experienced'}, \textit{`experienced'}, or \textit{`expert'} are classified as experienced users. 
% On the other hand, the participants who identified themselves as \textit{`somewhat experienced'}, \textit{`experienced'}, or \textit{`expert'} are classified as experienced users. 
% As stated in \textbf{H4}, we take both correctness score and completion time into account to verify if the novice users gained more performance boost using interactive contour-map than the experienced users. 
The sample ratio between these two groups was 1.06 which is fairly equal, as Fig. \ref{fig:demographic-data} suggests.





% \bgroup
% \def\arraystretch{1.2}%
\begin{table}[t]
% \small
\centering
\caption{Distribution of the 8 sets of tasks that account for the repetitive measures such as the spatial extent, visualization methods, and map layout. Each task set includes a task from the classification of the exploratory analysis tasks.}
% \begin{tabularx}{|c|l|c|c|}
% \begin{tabularx}{\columnwidth}{|X|X|X|X|}
\scriptsize
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{tabular} {P{2.5cm} | P{2.6cm} | P{1.1cm}| P{1.1cm}}
\hline
\textbf{Map Data Context} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Map Data\\ (Task Set)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Participant\\ Group 1\end{tabular}}                          & \textbf{\begin{tabular}[c]{@{}c@{}}Participant\\ Group 2\end{tabular}}                          \\ \hline
                                                                                                                              & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{T}1                                                                             & \cellcolor[HTML]{EFEFEF}                                                                         &                                                                                                 \\ 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Small Spatial Extent\\ (NY Temperature)\end{tabular}}                             & Multi Map - {[}D\textsubscript{T}2, D\textsubscript{T}3{]}                                                                    & \cellcolor[HTML]{EFEFEF}                                                                         &                                                                                                 \\ \cline{1-2}
\cellcolor[HTML]{EFEFEF}                                                                                                      & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{P}1                                                                             & \cellcolor[HTML]{EFEFEF}                                                                         &                                                                                                 \\ 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Large Spatial Extent\\ (CONUS Precipitation)\end{tabular}} & Multi Map - {[}D\textsubscript{P}2, D\textsubscript{P}3{]}                                                                    & \multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Static\\Maps\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Interactive\\Maps\end{tabular}}                    \\ \cline{1-2}
                                                                                                                              & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{T}4                                                                             &                                                                                                  & \cellcolor[HTML]{EFEFEF}                                                                        \\ 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Small Spatial Extent\\ (NY Temperature)\end{tabular}}                             & Multi Map - {[}D\textsubscript{T}5, D\textsubscript{T}6{]}                                                                    &                                                                                                  & \cellcolor[HTML]{EFEFEF}                                                                        \\ \cline{1-2}
\cellcolor[HTML]{EFEFEF}                                                                                                      & \cellcolor[HTML]{EFEFEF}Single Map - D\textsubscript{P}4                                                                             &                                                                                                  & \cellcolor[HTML]{EFEFEF}                                                                        \\
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Large Spatial Extent\\ (CONUS Precipitation)\end{tabular}} & Multi Map - {[}D\textsubscript{P}5, D\textsubscript{P}6{]}                                                                    & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Interactive\\Maps\end{tabular}}   & \multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Static\\Maps\end{tabular}} \\ \hline
\end{tabular}
\label{tab:task-distribution}
\end{table}



\subsection{Procedure}

Upon accessing the interface, the participants are first presented with an overview of the study, detailing the procedure, assignments, and the type of interaction data to be captured, culminating in a request for their consent. Subsequently, the interface collects basic demographic information from the participants such as level of education, gender, expertise with geospatial data analysis, familiarity with data visualization, and daily computer usage. %Next, the interface forwards the participants to a training window to describe the interactive features and familiarize them with the features in visual analysis. The training window includes 12 sections where we explain the contour map, geospatial data, and interactive features. % a couple of sample questions after providing detailed explanations for each interactive item to verify the participant's understanding. There is no pass or fail in the training phase. If participants select an incorrect answer, the interface interactively indicates the verdict and guides them to the correct answer. This interactive guidance and hints are predominantly implemented for the training and later disabled in the user study part. Once the training is complete, the interface will redirect the participant to the user study window.
The participants are then transitioned to a training session that introduces the interactive features for the purpose of visual exploration. 
% Participants are then transitioned to a training session that introduces them to the interactive features for visual analysis.
Across its 12 sections, the training modules elucidate the nuances of the contour map, the geospatial data, and the available interactive elements. To ensure comprehension, the participants encounter sample questions post each interactive feature's detailed explanation. 
% However, the training is not evaluative. 
Incorrect answers are met with on-screen guidance leading them to the correct response.
% This feedback mechanism is unique to the training phase and is deactivated during the actual user study. 
This feedback mechanism is unique to the training phase and is deactivated during the main session. 
Upon training completion, they are seamlessly moved to the main study session.  


In the main study session, the participants encounter 8 task sets (i.e., the second column in Table \ref{tab:task-distribution}), split into two distinct sections. Each set corresponds to a map layout showcasing different geospatial data. Within each set, there is a question representing each of the seven task types, culminating in a total of 56 questions (eight task sets $\times$ seven task questions) throughout the study. 
% In the user study, the interface prompts 8 sets of tasks (divided into two sections) where each set is associated with a map setup presenting different geospatial data. Each task set includes one question from each of the 7 task types which sum to 56 questions (8 $\times$ 7) for the study.
% Each section includes 4 sets of questions where two from temperature maps and two from precipitation maps. The questions in the two sections are identical where we change the map data for the following section to take the repetitive measures. For each participant, one of the sections is presented with a static map and another with an interactive map.
% To ensure counterbalancing, we divide our participants into two groups. One group answered from the static maps followed by the interactive maps and vice-versa for the other group. 
Table \ref{tab:task-distribution} provides a fair distribution of the map and task types, ensuring samples are counterbalanced and repetitive measures are taken into account. 
% \placeholder{The participants then submit results by selecting from the options provided for each task.}
The tasks are multiple choice type questions regarding the questions in Table~\ref{tab:exploratory-tasks}, and the participants can submit their answer by selecting from the options provided for each task. As participants perform the tasks, either by interacting or observing the map visualization, the interface logs their observations, task completion time (in seconds), and usage of any interactive features associated with questions. Upon completing the study, They get a completion code from the interface. They then submit the code to the MTurk portal to claim their incentive.

% To conduct this user intervention study, I am currently conducting a domain expert survey (discussed in section \ref{sec:domain-expert-survey}). Based on my obtained knowledge from the survey and literature reviews, I am in the process of creating a taxonomy of the analysis tasks that the scientists usually perform with the geospatial contours. In this user study, I will present several use cases for each of the analysis scenario. In each use cases, the participants will face a set of questions and interact with the prompted interactive geospatial visualization to answer. The interface will capture the participant's interaction with the interaction geospatial contours during the study. In addition, the interface stores participants answers along with the verdicts. The participants will answer different set of questions using both the interactive geospatial contour and static contour plots. Finally, the interface will prompt each participants a set of questionnaire to capture their impression on the interactive features for the geospatial contours.




\subsection{Evaluation Metrics}
Evaluating geospatial visualizations involves both qualitative and quantitative metrics \cite{tominski2011information}. 
In our study, we focus on quantitative metrics to evaluate the efficacy of interactive features embedded within the contour map. 
Roth \cite{roth2013empirically} described the objectives of cartographic interaction, to name a few, as (1) presenting insights preemptively, (2) coming to a decision point faster, meaning not solely doing it with a visual inspection. To assess the effectiveness of the interactive features in exploratory analysis tasks and validate our hypotheses, we focus on the  quantifiable factors - \textit{\textbf{task completion time}} and \textit{\textbf{the accuracy of their performed exploratory task -}} and \textit{\textbf{interaction logs during the task}}. The accuracy measures the participant's analytical ability to correctly answer the given multiple-choice questions. 

% \textbf{Dependent \& Independent Variables: } We consider two dependent variables: 1) task completion time, and 2) accuracy of the performed tasks. For the independent variables, we consider the interactive features on the map (visualization method) as discussed in Section \ref{sec:user-interactions}, and the exploratory task types as discussed in Section \ref{sec:task-specification}.
% By examining these factors, we aim to offer a robust quantitative analysis of map types (\textit{static vs. interactive}), and task types (\textit{7 exploratory data analysis tasks}). We also consider map layout (\textit{single vs. multi map}) and geospatial expertise (\textit{novice vs. experienced}) to analyze performance differences. 

% The performance metrics are designed to report a quantitative analysis that addresses the research questions stated in the earlier section.
% \textbf{Independent \& Dependent Variables: } For the independent variables, we considered the interactive features on the map and the exploratory task types. We considered two dependent variables: 1) task completion time, and 2) correctness of the performed tasks. 

% \subsection{Analysis Methods}
% We intend to utilize the user interaction data to evaluate the task completion time. The setup and procedures of the user intervention study is outlined in section \ref{sec:user-intervention-study} later. 
% \IC{we just need to mention what method we used for analysis.}
% We leverage two-way and one-way repeated measures analysis of variance (ANOVA) at a 95\% confidence level as our primary method to test the effect of the independent variables on different exploratory task types. 

\subsection{Hypotheses} \label{sec:hypothesis-rq}
% Acknowledging the potential of interactive contours in a geospatial view for visually analyzing high-resolution geospatial data, it is essential to understand the utility of interactive features to the full extent. %The core research question of this work is, ``Can interactive geospatial maps improve users' exploratory visual analytic capabilities?'
% To address our RQs in
% Section 1, we establish the following hypotheses for our study:

Acknowledging the potential of interactive contours in a geospatial view for visually analyzing geospatial data, it is essential to understand the utility of interactive features to the full extent. %The core research question of this work is, ``Can interactive geospatial maps improve users' exploratory visual analytic capabilities?'
To address our RQs in Section 1, we establish the following hypotheses for our study:


% \begin{enumerate}
% [label=\textbf{RQ\arabic*.}]
    % \item[RQ1.] Do interactive features in the geospatial map improve the usability over static map in visually extracting information?
    % \textbf{RQ1.} Do interactive contour maps enhance users' performance in visually conducting exploratory analytical tasks, both in terms of accuracy in their estimations and the time taken to complete these tasks?
    % \textbf{RQ1.} Do interactive contour maps enhance users' performance in visually conducting exploratory analytical tasks, both in terms of estimation accuracy and task completion time?

    \begin{enumerate}[label=\textbf{H\arabic*:}]
    \item Interactive features can improve users' accuracy when performing exploratory geospatial analysis tasks. % However, because of the additional interactive features and associated cognitive processing, users might need more time to complete tasks.
    
    % \textbf{RQ2.} Do the interactive features on the map significantly outperform static maps in aiding users during various exploratory analysis tasks?
    % \textbf{RQ2.} Do the interactive features significantly outperform static maps in aiding users during various exploratory analysis tasks?
    
    \item When the interactive features are available, users might need more time to complete tasks \HDY{compared to using} the static map due to associated cognitive processing.
    
    % \item Interactive maps improve users' performance in complex exploratory analysis tasks compared to static maps. Users are expected to perform better in tasks that involve discerning relationships among multiple data points or contour regions. While users may spend more time completing the tasks to achieve higher accuracy in exploration, the overall individual performance, in terms of accuracy per time, is expected to improve significantly. 
% \end{enumerate}

    % \item Interactive maps enhance performance for novice users unfamiliar with geospatial analysis, more than they do for experienced users. While performance metrics include both accuracy and task completion time, experienced users are anticipated to outperform novice users in accuracy. However, interactive maps could lead novice users to an improved accuracy per time, implying that the time spent interacting with the map would be more beneficial for them compared to experienced users in geospatial analysis.

    % \item Comparative exploration between multiple maps is expected to be more challenging than exploring a single map \placeholder{because ...}

    \item When two maps are presented, interactive features of synchronization could offer the potential to improve accuracy in multiple map exploration tasks. 

    

\end{enumerate}

%Participants will be presented with multiple question sets derived from different geospatial contour maps. The contour maps are divided into two groups where one group is presented with the interactive features and others with the static illustrations. 


    % We leveraged a taxonomy of exploratory geospatial analysis for task design (detailed further in Section \ref{sec:task-specification}).

% We leveraged a taxonomy of exploratory geospatial analysis for task design in Section \ref{sec:task-specification}. We then outlined potential workflows in the context of visual analysis. Participants will be presented with multiple sets of unique analysis tasks from the classification. The tasks in a set are designed around a contour map and provide the full extent of interactive features to trial with a group of participants. Another group performed similar tasks with the static version of the same contour maps. 

% We measure the likeliness of utilizing each individual interactive feature in different exploratory analysis tasks. We report the usage of the interactive features and analyze the underlying patterns in the usage. These patterns are quantified based on the time differential of performing the tasks and their usage sequence.
% To report answers for these research questions, we have designed a comparative user intervention study. We outline following hypotheses and quantitatively justify our claim analyzing the data collected from the crowd-sourced user study:
% \begin{enumerate}
% [label=H\arabic*.]
%     % \item Interactive features in geospatial contour benefit users in better performing exploratory analysis tasks - 1) Task completion time, 2) Task precision/correctness
%     % \item A quantitative evaluation would be essential to identify the interactive features that are useful for the contour-based exploratory analysis.
%     \item A quantitative analysis that creates a one-to-many mapping between the analysis tasks and interactive features can benefit visualization researchers in the future to explore task-specific interactive contour maps.

% \end{enumerate}


\section{Results}
% We leverage two-way and one-way repeated measures analysis of variance (ANOVA) at a 95\% confidence level. 
% We leverage two-way repeated measures analysis of variance (ANOVA) at a 95\% confidence level. 
% The two-way ANOVA evaluates performance metrics based on map and task types. 
% To present the estimates, we also report the lower and upper bounds at a 95\% confidence interval (CI). To present differences between visualization methods, we report the $p$-value and the error bound mean ($EBM$) for the task types. 
% Furthermore, we provide a quantitative ranking of the usability of interactive features within the visual analytics interface for the participating task types. We expect that it would be beneficial for visualization researchers in the future to employ different interactive features based on the intended analysis tasks.

We leverage two-way repeated measures analysis of variance (ANOVA) at a 95\% confidence level. It evaluates performance metrics based on the map types (interactive vs. static) and map layouts (single map vs. multi map) across the task types. Although our results violate the normality test, we use ANOVA because the previous study~\cite{blanca2017non} provided empirical evidence for its robustness when evaluating data with non-normal distributions. To present the estimates, we also report the lower and upper bounds at a 95\% confidence interval (CI). To present differences between visualization methods, we report the $p$-value and the error bound mean ($EBM$) for the task types. 
% We leverage three-way repeated measures analysis of variance (ANOVA) at a 95\% confidence level. It evaluates performance metrics based on map types, map layouts, and task types. To present the estimates, we also report the lower and upper bounds at a 95\% confidence interval (CI). To present differences between visualization methods, we report the $p$-value and the error bound mean ($EBM$) for the task types. 


% Analyzing the interaction data to calculate the z-score would help to understand the potential of interactive visualizations in exploratory analysis of geospatial data. 
% In statistical analysis, z-score describes a position of a value in compared to a group of scores. The z-score becomes 0 if the data value is identical to the group's mean score. In contrast, z-score of 1 indicates the value is one standard deviation from the group's mean score. The z-score can be positive or negative depending on the value's position above or below the mean score. The z-score can be computed using the following formula: \[Z = \frac{x - \mu}{\sigma}\] Where $x$ is the observed value, $\mu$ is mean of the sample scores, and $\sigma$ is the standard deviation of the samples. 
% T-test is an inferential statistical technique to determine the existing difference between to independent group of scores. Applying t-test in the quantitative analysis would provide a validation to the proposed hypothesis for the visual analytics interface in comparison to the traditional spatiotemporal data analysis methods. 
% \[t = \frac{M\textsubscript{2} - M\textsubscript{1}}{\sqrt{\frac{s\textsubscript{1}^2}{n\textsubscript{1}} + \frac{s\textsubscript{2}^2}{n\textsubscript{2}}}}\]
% Where M\textsubscript{1} and M\textsubscript{2} denotes sample means, s\textsubscript{1} and s\textsubscript{2} are sample variances, and n\textsubscript{1}, n\textsubscript{2} denotes two individual group of samples. 
% Moreover, we included another statistical technique, Analysis of Variance (ANOVA) \cite{st1989analysis}, to evaluate the interactive map in terms of accuracy of visual estimation while performing analysis tasks. 
% ANOVA helps to find the statistical differences among the means of two or more group of scores. 

==> sections/Prev/7-results__old_2_.tex <==
%  descriptive analysis in result section

% In this section, we apply statistical analysis methods to testify our hypothesis in order to validate the research questions raised in Section \ref{sec:hypothesis-rq}. 
% To test the hypotheses, we have considered two measures from data collected in the user study: the correctness of the analysis tasks and task completion time. Correctness is measured based on the participant's ability to estimate the correct answer from the options. Additionally, the user interface tracked the time elapsed before the participants completed each task.

% \bgroup
% \def\arraystretch{1.2}%
% \begin{table}[t]
% \centering
% % \tiny
% \caption{Two-way ANOVA results for accuracy and task completion time required with visualization methods (static vs. interactive maps) and exploratory task types.}
% \small
% \begin{tabular}{ | p {0.5em} | p {8em} |  p {7em} | p {3.1em} | p {2em} | }
% % \begin{tabularx}{\columnwidth}{|X|X|X X|X|X|}
% % .                        & Factors                          & MS         & F       & P     & np2   \\
% \hline
% -                             &\textbf{Factor}             & \textbf{\textit{F}} & \textbf{$p$} & \textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}} \\ \hline
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize{Accuracy}                     }}  & \cellcolor[HTML]{EFEFEF}Map Type $\times$ Task      & \cellcolor[HTML]{EFEFEF}(6, 366)=2.908  & \cellcolor[HTML]{EFEFEF}\textbf{.006} & \cellcolor[HTML]{EFEFEF}.046 \\
%                               & Map Type                & (1, 61)=114.186 & \textless\textbf{.001} & .652 \\
%                               & \cellcolor[HTML]{EFEFEF}Task                           & \cellcolor[HTML]{EFEFEF}(6, 366)=107.459 & \cellcolor[HTML]{EFEFEF}\textless\textbf{.001} & \cellcolor[HTML]{EFEFEF}.638 \\ \hline\hline
% \multirow{3}{*}{\rotatebox[origin=c]{90}{Time                    }} & \cellcolor[HTML]{EFEFEF}Map Type $\times$ Task &  \cellcolor[HTML]{EFEFEF}(6, 366)=.892   & \cellcolor[HTML]{EFEFEF}.513 & \cellcolor[HTML]{EFEFEF}.015 \\
%                               & Map Type            & (1, 61)=5.755   & \textbf{.020} & .088 \\
%                               & \cellcolor[HTML]{EFEFEF}Task                      & \cellcolor[HTML]{EFEFEF}(6, 366)=7.698   & \cellcolor[HTML]{EFEFEF}\textless\textbf{.001} & \cellcolor[HTML]{EFEFEF}.114 \\
% \hline
% \end{tabular}
% \label{tab:task-method-table}
% \end{table}
% \begin{tabular}{ | p {0.5em} | p {5em} | h | p {7em} | p {3.1em} | p {2em} | }
% % \begin{tabularx}{\columnwidth}{|X|X|X X|X|X|}
% % .                        & Factors                          & MS         & F       & P     & np2   \\
% \hline
% -                             &\textbf{Factor}             & \textbf{\textit{DoF}} & \textbf{\textit{F}} & \textbf{$p$} & \textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}} \\ \hline
% \multirow{3}{*}{\rotatebox[origin=c]{90}{Accuracy                     }}  & Vis $\times$ Task & 6      & (6, 366)=2.908  & \textbf{.006} & .046 \\
%                               & Vis             & 1     & (1, 61)=114.186 & < \textbf{.001} & .652 \\
%                               & Task                       & 6     & (6, 366)=107.459 & < \textbf{.001} & .638 \\ \hline
% \multirow{3}{*}{\rotatebox[origin=c]{90}{Time                    }} & Vis $\times$ Task & 6 & (6, 366)=.892   & .513 & .015 \\
%                               & Vis             & 1 & (1, 61)=5.755   & \textbf{.020} & .088 \\
%                               & Task                      & 6 & (6, 366)=7.698   & <\textbf{.001} & .114 \\
% \hline
% \end{tabular}
% \label{tab:task-method-table}
% \end{table}

% \subsection{Effect of User Interactions}
% The statistical results for interaction and main effects of map types and tasks are presented in Table \ref{tab:task-method-table}. 
% A significant interaction effect on the overall achieved task accuracy ($p=.006$) between the map and task types is disclosed. However, we find no interaction effect on the task completion time ($p=.513$). For details about their simple effects, please refer to the following section. 




% \begin{figure}[t]
%     \centering
%     % \setlength{\abovecaptionskip}{-3pt}
%     % \setlength{\belowcaptionskip}{-10pt}

%     \includegraphics[width=0.9\linewidth]{figures/overall-performance-updated.png}
%     \caption{
%       The results of overall accuracy and task completion time with 95\% CI. 
%     }
%     \label{fig:overall-performance-error-plot}
% \end{figure}


% The significant main effects of the map type ($p<.001$) and the task type ($p<.001$) on the overall accuracy are reported. Fig. \ref{fig:overall-performance-error-plot}-A shows the overall accuracy with its 95\% CI by the map type. 
% Interactive geospatial maps ($M=.65$, $EBM=[.62, .68]$) evidently assist in better accuracy than static maps ($M=.54$, $EBM=[.51, .56]$). 
% We also discovered a significant main effect of map type on task completion time, indicating that participants spent more time with interactive maps ($M=16.06 min$, $EBM=[12.63, 19.49]$) than static maps ($M=12.34 min$, $EBM=[10.01, 14.66]$) . The results is shown in Fig. \ref{fig:overall-performance-error-plot}-B.

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
% \tiny
\small
\caption{Accuracy and completion time results of the tasks from exploratory task types using the static and interactive maps.}
\begin{tabularx}{\columnwidth}{X|XXX|XXX|}
\cline{2-7} & \multicolumn{3}{c|}{\textbf{Accuracy}}                   & \multicolumn{3}{c|}{\textbf{Completion Time}}     \\ \hline
\multicolumn{1}{|l|}{\textbf{Task Type}}                  & \textbf{F(1,61)} & \textbf{\textit{p}}              & \textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}} & \textbf{F(1,61)} & \textbf{\textit{p}}    & \textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Associate}   & \cellcolor[HTML]{EFEFEF}24.257             & \cellcolor[HTML]{EFEFEF}\textbf{\textless .001} & \cellcolor[HTML]{EFEFEF}.285         & \cellcolor[HTML]{EFEFEF}5.988              & \cellcolor[HTML]{EFEFEF}\textbf{.017} & \cellcolor[HTML]{EFEFEF}.091         \\
\multicolumn{1}{|l|}{Categorize}  & 13.897             & \textbf{\textless .001} & .186         & 8.601              & \textbf{.005} & .125         \\
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Cluster}     & \cellcolor[HTML]{EFEFEF}20.902             & \cellcolor[HTML]{EFEFEF}\textbf{\textless .001} & \cellcolor[HTML]{EFEFEF}.255         & \cellcolor[HTML]{EFEFEF}2.436              & \cellcolor[HTML]{EFEFEF}.124          & \cellcolor[HTML]{EFEFEF}.039         \\
\multicolumn{1}{|l|}{Distinguish} & 2.531              & .117                    & .042         & 2.750              & .102          & .044         \\
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Identify}    & \cellcolor[HTML]{EFEFEF}4.923              & \cellcolor[HTML]{EFEFEF}\textbf{.030}           & \cellcolor[HTML]{EFEFEF}.075         & \cellcolor[HTML]{EFEFEF}8.263              & \cellcolor[HTML]{EFEFEF}\textbf{.006} & \cellcolor[HTML]{EFEFEF}.121         \\
\multicolumn{1}{|l|}{Locate}      & 3.279              & .058                    & .058         & .839               & .363          & .014         \\
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Rank}        & \cellcolor[HTML]{EFEFEF}9.445              & \cellcolor[HTML]{EFEFEF}\textbf{.003}           & \cellcolor[HTML]{EFEFEF}.134         & \cellcolor[HTML]{EFEFEF}.018               & \cellcolor[HTML]{EFEFEF}.893          & \cellcolor[HTML]{EFEFEF}.000         \\ \hline
\end{tabularx}
\label{tab:task-wise-performance}
\end{table}

\subsection{User Interaction Effect on Exploratory Tasks}

% To test \textbf{H2}, we report statistical results of the performance metrics in terms of the interactive features by tasks. 
Table \ref{tab:task-wise-performance} and Fig. \ref{fig:performance-ci} show the statistical results of the simple effects of the task types. 

\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    % \includegraphics[width=\linewidth]{figures/performance-ci-updated.pdf}
    \includegraphics[width=\linewidth]{figures/performance-ci-dy.png}
    \caption{
    The results of accuracy and task completion time by tasks and map types; 
    % The participants' error bound mean ($EBM$) accuracy and task completion times. 
    While the completion time is often faster with the static maps, the accuracy is consistently better with the interactive maps.
      }
    \label{fig:performance-ci}
    \vspace{-.5cm}
\end{figure}

{\textbf{Associate:} The accuracy shows a significant difference between the static and interactive maps ($p<.001$).
The task accuracy suggests that the participants performed substantially better using the interactive map ($M=.46$, $EBM=[.41, .52]$) compared to the static map ($M=.29$, $EBM=[.25, .34]$). 
We also find a significant difference in the completion time between the map types ($p=.017$).
The participants spent statistically more time on the interactive map ($M=125.24 s$, $EBM=[91.44, 159.04]$) than the static map ($M=91.67 s$, $EBM=[68.68, 114.67]$).


\textbf{Categorize:} The map types show significant differences in terms of accuracy ($p<.001$) and completion time ($p<.001$). 
The accuracy in the interactive map ($M=.58$, $EBM=[.51, .65]$) is statistically higher than the static map ($M=.43$, $EBM=[.38, .49]$) in performing the categorize-type tasks. 
However, the interactive map condition ($M=196.74s$, $EBM=[147.91, 245.52]$) takes more time than the static map condition ($p=.005$, $M=138.50s$, $EBM=[110.31, 166.70]$). 

\textbf{Cluster:} A statistical difference in accuracy between the map types is reported ($p<.001$). 
Its pairwise comparison result shows that the interactive map ($M=.56$, $EBM=[.49, .64]$) supported the participants better than the static map ($M=.36$, $EBM= [.30, .43]$). 
% No statistical difference in task completion time between map types ($p=.124$) is found. 


% \textbf{Distinguish} 
% The difference in accuracy ($p=.117$) and task completion time ($p=.102$) are statistically insignificant between the static and interactive map types.

\textbf{Identify:}
The accuracy results illustrate a significant difference between the map types ($p=.030$). 
The posthoc test reveals the participants achieved better results with the interactive map ($M=.52$, $EBM=[.45, .59]$) compared to the static map ($M=.42$, $EBM=[.35, .48]$). 
The task completion time difference is also statistically significant between the map types ($p=.006$). The participants spent more time in the interactive map condition ($M=114.39 s$, $EBM=[88.46, 140.32]$) than the static map condition ($M=90.07 s$, $EBM=[69.62, 110.52]$).

% \textbf{Locate:}
% The participants' task accuracy ($p=.058$) and task completion time ($p=.363$) show no significant differences between the map types.

\textbf{Rank:}
We observe a significant difference ($p=.003$) in the accuracy between the map types. 
The interactive map ($M=.73$, $EBM=[.67, .79]$) has a higher accuracy than the static map ($M=.60$, $EBM=[.53, .67]$). 
% However, no difference in the task completion time between the map types ($p=.893$) is disclosed.


\textbf{Distinguish \& Locate:} No clear difference in terms of accuracy and task completion time is disclosed.

% \textbf{In summary,} these findings support our \textbf{H1} and \textbf{H2} that interactive maps help users produce more accurate results while taking longer to complete tasks.
\textbf{In summary,} \HDY{these findings partially support our \textbf{H1} and \textbf{H2}. We found that the accuracy could be significantly improved using interactive features for five out of seven tasks (i.e., Associate, Categorize, Cluster, Identify, and Rank). Despite the performance enhancements offered by the interactive features, we observed no noticeable variation in completion time for the Cluster and Rank tasks. However, the Associate, Categorize, and Identity tasks exhibited longer durations. }
% It suggest that interactive maps for  could help users produce more accurate results while taking longer to complete tasks.

\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[width=\linewidth]{figures/single-vs-multiple-dy.png}
    \caption{Accuracy comparison between single and multi-maps using static (left) and interactive (right) geospatial visualization. 
    % \placeholder{need to update}
    }
    \label{fig:single-multiple-performance-ci}
\end{figure}


\subsection{\placeholder{User Interaction Effect on Multi-maps Exploration}}
\HDY{HDY: need to update} This section reports the interaction effect of map layouts by map and task types on accuracy ($p=.038$). 
The accuracy results by the factors are shown in Fig. \ref{fig:single-multiple-performance-ci}. 
% We discovered a small number of factor combinations with significant differences. 
For the associate task, the static map condition shows significantly different accuracy ($p=.001$) between the single ($M=.19$, $EBM=[.12, .27]$) and multi map conditions ($M=.40$, $EBM=[.31, .48]$). However, the interactive map condition shows no difference ($p=0.715$) between the single ($M=.45$, $EBM=[.36, .55]$) and multi maps ($M=.48$, $EBM=[.38, .57]$). 
% The result suggests that the interactive map condition narrowed down the accuracy gaps to a slender margin between single and multi-map exploration (\textbf{H3}). 
The cluster task shows statistically different accuracy for the static map condition ($p=.017$), while the interactive map condition does not ($p=.368$). However, we found no significant main effect of map layout on accuracy  ($p=.513$).
% The results disclose that the accuracy using the single map ($M=1.032$, $EBM=[.353, 1.872]$) is significantly higher than the multi-map condition ($M=.694$, $EBM=[.114, 1.459]$).

\textbf{In summary,} \HDY{the results do not directly support our \textbf{H3}. However, they suggest that the interactive map condition narrowed down the accuracy gaps to a slender margin between single and multi-map exploration.}

% The accuracy results are shown in Fig. \ref{fig:single-multiple-performance-ci}. 
% For the associate task, the static map condition shows significantly different accuracy ($p=.001$) between the single ($M=.79$, $EBM=[.20, 1.563]$) and multi map conditions ($M=.39$, $EBM=[.091, 1.099]$). However, the interactive map condition shows no difference ($p=0.715$) between the single ($M=.952$, $EBM=[.327, 1.819]$) and multi maps ($M=.903$, $EBM=[.256, 1.72]$). 
% The result suggests that the interactive map condition narrowed down the accuracy gaps to a slender margin between single and multi-map exploration (\textbf{H3}). 
% The cluster task shows statistically different accuracy for the static map condition ($p=.017$), while the interactive map condition does not ($p=.368$).
% The results disclose that the accuracy using the single map ($M=1.032$, $EBM=[.353, 1.872]$) is significantly higher than the multi-map condition ($M=.694$, $EBM=[.114, 1.459]$).

% , supporting \textbf{H3}. 
% The cluster (static $p=.017$; interactive $p=.368$) and rank tasks (static $p=.023$; interactive $p=.125$) showed similar results on the accuracy. 
% For example, the accuracy for the cluster task using the single map ($M=1.032$, $EBM=[.353, 1.872]$) was 
% whereas, in interactive maps the difference between single ($M=1.194$, $EBM=[.590, 1.979]$) and multi-maps ($M=1.065$, $EBM=[.262, 2.046]$) are insignificant.
% Though we find no significant accuracy difference between the map types, the tasks of identify, locate, and rank showed a similar but weak tendency, except for the distinguish-type task.
% Similar to the cluster task, the single map had a higher  accuracy than the multi-map in the identify, locate, and rank tasks. 
% Similar to the cluster task, the single map had a higher  accuracy than the multi-map in the identify ($MD=-.21$), locate ($MD=-.23$), and rank ($MD=-.29$) tasks. 
% For example, in the rank task, the accuracy difference between single ($M=1.371$, $EBM=[.821, 2.105]$) and multi-maps ($M=1.548$, $EBM=[1.016, 2.312]$) was insignificant ($p$=\placeholder{X}) in interactive maps, however, for both static and interactive maps, the participants performed better in the multi-maps compared to the single maps. 
% Regardless of the performance gap between single and multi-maps, the participants' correctness score improved in all task types in interactive maps, except for the distinguish-type tasks. 
% Interestingly, however, the accuracy using the single map ($M=1.032$, $EBM=[.353, 1.872]$) is significantly higher than the multi-map condition ($M=.694$, $EBM=[.114, 1.459]$).
% These findings partially reaffirm both the hypotheses \textbf{H2} and \textbf{H3}.



% The accuracy results are shown in Fig. \ref{fig:single-multiple-performance-ci}. 
% % For the associate task in static maps, the correctness difference between single ($M=.790$, $EBM=[.20, 1.563]$) and multi-maps ($M=.387$, $EBM=[.091, 1.099]$) is significant ($p=.001$) whereas, in interactive maps, the difference becomes insignificant ($p=0.715$) between single ($M=.952$, $EBM=[.327, 1.819]$) and multi-maps ($M=.903$, $EBM=[.256, 1.72]$). 
% For the associate task, the static map condition shows significantly different accuracy ($p=.001$) between the single ($M=.790$, $EBM=[.20, 1.563]$) and multi map conditions ($M=.387$, $EBM=[.091, 1.099]$), supporting \textbf{H3}. However, the interactive map condition shows no difference ($p=0.715$) between the single ($M=.952$, $EBM=[.327, 1.819]$) and multi maps ($M=.903$, $EBM=[.256, 1.72]$). 
% The result suggests that the interactive map condition narrowed down the accuracy gaps to a slender margin between single and multi-map exploration (\textbf{H4}). 
% The cluster task shows statistically different accuracy for the static map condition ($p=.017$), while the interactive map condition does not ($p=.368$).
% % The cluster (static $p=.017$; interactive $p=.368$) and rank tasks (static $p=.023$; interactive $p=.125$) showed similar results on the accuracy. 
% % For example, the accuracy for the cluster task using the single map ($M=1.032$, $EBM=[.353, 1.872]$) was 
% % whereas, in interactive maps the difference between single ($M=1.194$, $EBM=[.590, 1.979]$) and multi-maps ($M=1.065$, $EBM=[.262, 2.046]$) are insignificant.
% Though we find no significant accuracy difference between the map types, the tasks of identify, locate, and rank showed a similar but weak tendency, except for the distinguish-type task.
% % Similar to the cluster task, the single map had a higher  accuracy than the multi-map in the identify, locate, and rank tasks. 
% % Similar to the cluster task, the single map had a higher  accuracy than the multi-map in the identify ($MD=-.21$), locate ($MD=-.23$), and rank ($MD=-.29$) tasks. 
% % For example, in the rank task, the accuracy difference between single ($M=1.371$, $EBM=[.821, 2.105]$) and multi-maps ($M=1.548$, $EBM=[1.016, 2.312]$) was insignificant ($p$=\placeholder{X}) in interactive maps, however, for both static and interactive maps, the participants performed better in the multi-maps compared to the single maps. 
% % Regardless of the performance gap between single and multi-maps, the participants' correctness score improved in all task types in interactive maps, except for the distinguish-type tasks. 
% Interestingly, however, the accuracy using the single map ($M=1.032$, $EBM=[.353, 1.872]$) is significantly higher than the multi-map condition ($M=.694$, $EBM=[.114, 1.459]$).
% These findings partially reaffirm both the hypotheses \textbf{H2} and \textbf{H3}.


==> sections/Prev/7-results_old_.tex <==

% \begin{table}[t]
% \centering
% % \tiny
% \small
% \caption{Accuracy and completion time results of the tasks from exploratory task types using the static and interactive maps.}
% \begin{tabularx}{\columnwidth}{X|XXX|XXX|}
% \cline{2-7} & \multicolumn{3}{c|}{\textbf{Accuracy}}                   & \multicolumn{3}{c|}{\textbf{Completion Time}}     \\ \hline
% \multicolumn{1}{|l|}{\textbf{Task Type}}                  & \textbf{F(1,61)} & \textbf{\textit{p}}              & \textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}} & \textbf{F(1,61)} & \textbf{\textit{p}}    & \textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}} \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Associate}   & \cellcolor[HTML]{EFEFEF}24.257             & \cellcolor[HTML]{EFEFEF}\textbf{\textless .001} & \cellcolor[HTML]{EFEFEF}.285         & \cellcolor[HTML]{EFEFEF}5.988              & \cellcolor[HTML]{EFEFEF}\textbf{.017} & \cellcolor[HTML]{EFEFEF}.091         \\
% \multicolumn{1}{|l|}{Categorize}  & 13.897             & \textbf{\textless .001} & .186         & 8.601              & \textbf{.005} & .125         \\
% \multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Cluster}     & \cellcolor[HTML]{EFEFEF}20.902             & \cellcolor[HTML]{EFEFEF}\textbf{\textless .001} & \cellcolor[HTML]{EFEFEF}.255         & \cellcolor[HTML]{EFEFEF}2.436              & \cellcolor[HTML]{EFEFEF}.124          & \cellcolor[HTML]{EFEFEF}.039         \\
% \multicolumn{1}{|l|}{Distinguish} & 2.531              & .117                    & .042         & 2.750              & .102          & .044         \\
% \multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Identify}    & \cellcolor[HTML]{EFEFEF}4.923              & \cellcolor[HTML]{EFEFEF}\textbf{.030}           & \cellcolor[HTML]{EFEFEF}.075         & \cellcolor[HTML]{EFEFEF}8.263              & \cellcolor[HTML]{EFEFEF}\textbf{.006} & \cellcolor[HTML]{EFEFEF}.121         \\
% \multicolumn{1}{|l|}{Locate}      & 3.279              & .058                    & .058         & .839               & .363          & .014         \\
% \multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Rank}        & \cellcolor[HTML]{EFEFEF}9.445              & \cellcolor[HTML]{EFEFEF}\textbf{.003}           & \cellcolor[HTML]{EFEFEF}.134         & \cellcolor[HTML]{EFEFEF}.018               & \cellcolor[HTML]{EFEFEF}.893          & \cellcolor[HTML]{EFEFEF}.000         \\ \hline
% \end{tabularx}
% \label{tab:task-wise-performance}
% \end{table}



\subsection{Accuracy}

Fig. \ref{fig:performance-ci} shows the accuracy results by task types, and map types and layouts. 


\hspace{\parindent}\textbf{Associate:} %No interaction effect was reported between map type and layout ($p=.082$, $F(1, 61)=3.127$, $\eta^2_p=.049$). 
Main effects of map type ($p<.001$, $F(1, 61)=24.362$, $\eta^2_p=.285$) and layout ($p=.017$, $F(1, 61)=6.015$, $\eta^2_p=.090$) were disclosed. The task accuracy suggests that the participants performed substantially better using the interactive map ($M=.460$, $EBM=[.403, .516]$) compared to the static map ($M=.294$, $EBM=[.247, .341]$). We also find the participants performed the task more accurately when they used multi-map ($M=.431$, $EBM=[.367, .500]$) than the single-map ($M=.323$, $EBM=[.268, .377]$).


\textbf{Categorize:} %We found no interaction effect ($p=.666$, $F(1, 61)=.188$, $\eta^2_p=.003$), but
We found main effects of map type ($p<.001$, $F(1, 61)=13.897$, $\eta^2_p=.186$) and map layout ($p<.001$, $F(1, 61)=13.346$, $\eta^2_p=.180$). \HDY{The accuracy when using the interactive map ($M = .581$, $EBM = [.509, .652]$) is statistically higher than when using the static map ($M = .431$, $EBM = [.376, .487]$) for categorize-type tasks.}
% The accuracy in the interactive map ($M=.581$, $EBM=[.509, .652]$) is statistically higher than using the static map ($M=.431$, $EBM=[.376, .487]$) in performing the categorize-type tasks.
Next, the multi-map condition ($M=.581$, $EBM=[.518, .643]$) showed higher accuracy than the single-map condition ($M=.431$, $EBM=[.365, .498]$).


\textbf{Cluster:} The map type ($p<.001$, $F(1, 61)=19.973$, $\eta^2_p=.247$) and map layout ($p=.036$, $F(1, 61)=4.611$, $\eta^2_p=.070$) showed main effects. %while there was no interaction effect ($p=.305$, $F(1, 61)=1.072$, $\eta^2_p=.017$). 
Regarding the map type, its pairwise comparison result shows that the interactive map ($M=.560$, $EBM=[.491, .630]$) supported the participants better than the static map ($M=.363$, $EBM= [.297, .429]$). The multi-map condition ($M=.520$, $EBM=[.455, .585]$) showed higher accuracy than the single-map condition ($M=.403$, $EBM=[.320, .486]$).


\textbf{Distinguish:} An interaction effect between the map type and layout was found ($p=.015$, $F(1, 61)=6.295$, $\eta^2_p=.094$). We found a simple effect of the map type when the map layout is multi-map ($p=.002$, $F(1, 61)=10.738$, $\eta^2_p=.150$). Its post-hoc test showed the interactive map ($M=.629$, $EBM=[.553, .705]$) has higher accuracy than the static map ($M=.444$, $EBM=[.354, .533]$).

We found a main effect of map layout ($p=.022$, $F(1, 61)=5.544$, $\eta^2_p=.083$) but not map type ($p=.117$, $F(1, 61)=2.531$, $\eta^2_p=.040$). The pairwise comparison showed the multi-map condition ($M=.536$, $EBM=[.476, .597]$) showed higher accuracy than the single-map condition ($M=.435$, $EBM=[.372, .499]$).


\textbf{Identify:} %No interaction effect was disclosed ($p=.220$, $F(1, 61)=1.536$, $\eta^2_p=.025$). However, 
Main effects of map type ($p=.030$, $F(1, 61)=4.923$, $\eta^2_p=.075$) and map layout ($p<.001$, $F(1, 61)=12.219$, $\eta^2_p=.167$) were revealed. The posthoc test revealed \HDY{that} the participants achieved better results with the interactive map ($M=.516$, $EBM=[.444, .588]$) compared to the static map ($M=.415$, $EBM=[.355, .476]$). It also found the participant with the single-map condition ($M=.544$, $EBM=[.480, .609]$) had higher accuracy than the multi-map condition ($M=.387$, $EBM=[.319, .455]$).


\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    % \includegraphics[width=\linewidth]{figures/performance-ci-updated.pdf}
    \includegraphics[width=\linewidth]{figures/accuracy-result-2024-2.png}
    \caption{
    % The results of accuracy and task completion time by tasks and map types; 
    The accuracy results by tasks, map types, and map layouts 
    % The participants' error bound mean ($EBM$) accuracy and task completion times. 
    % While the completion time is often faster with the static maps, the accuracy is consistently better with the interactive maps.
      }
    \label{fig:performance-ci}
    % \vspace{-.5cm}
\end{figure}
\textbf{Locate:} We only found a main effect of map layout ($p=.002$, $F(1, 61)=10.333$, $\eta^2_p=.145$). Its pairwise comparison showed the multi-map condition ($M=.835$, $EBM=[.767, .903]$) showed higher accuracy than the single-map condition ($M=.710$, $EBM=[.643, .776]$).


\textbf{Rank:} We discovered the main effects of map type ($p=.003$, $F(1, 61)=9.445$, $\eta^2_p=.134$) and map layout ($p<.001$, $F(1, 61)=15485$, $\eta^2_p=.202$).%, but no interaction effect ($p=.539$, $F(1, 61)=.382$, $\eta^2_p=.006$). 
The interactive map ($M=.730$, $EBM=[.669, .791]$) has a higher accuracy than the static map ($M=.597$, $EBM=[.527, .667]$). The single-map ($M=.722$, $EBM=[.668, .776]$) has a higher accuracy than the multi-map ($M=.605$, $EBM=[.543, .666]$).


\subsection{Task Completion Time}
Fig. \ref{fig:single-multiple-performance-ci} shows the task completion time results by task types, and map types and layouts. 

\hspace{\parindent}\textbf{Associate:} We found no interaction effect ($p=.102$, $F(1, 61)=2.761$, $\eta^2_p=.043$), but found main effects of map type ($p=.016$, $F(1, 61)=6.091$, $\eta^2_p=.091$) and map layout ($p=.019$, $F(1, 61)=5.849$, $\eta^2_p=.087$). 
The pairwise comparison results for the map type showed the participants spent statistically more time on the interactive map ($M=62.188s$, $EBM=[45.547, 78.829]$) than the static map ($M=45.535s$, $EBM=[34.210, 56.859]$). Next, we also found the participants spent more time on the multi-map condition ($M=60.175s$, $EBM=[45.053, 75.298]$) than single-map ($M=47.547s$, $EBM=[35.716, 59.378]$).


\textbf{Categorize:} We found a main effect of map type ($p=.005$, $F(1, 61)=8.480$, $\eta^2_p=.122$). Its pairwise comparison disclosed that the interactive map condition ($M=98.020s$, $EBM=[74.024, 122.017]$) takes more time than the static map condition ($M=69.519s$, $EBM=[55.645, 83.392]$). 

% \textbf{Cluster:} No clear difference in task completion time is disclosed by the task type and layout.

\textbf{Distinguish:} A main effect of map layout ($p=.026$, $F(1, 61)=5.236$, $\eta^2_p=.079$) was reported. Its pairwise comparison disclosed that the single-map condition ($M=47.473s$, $EBM=[37.381, 57.565]$) takes more time than the multi-map condition ($M=38.201s$, $EBM=[29.710, 46.692]$). 

\textbf{Identify:} The task completion time difference is statistically significant between the map types ($p=.023$). The participants spent more time in the interactive map condition ($M=58.340s$, $EBM=[45.385, 71.296]$) than the static map condition ($M=47.859s$, $EBM=[36.327,59.392]$).

\textbf{Cluster, Locate, \& Rank:} No clear difference in task completion time is disclosed by the task type and layout.


% \textbf{Rank:}





% To test \textbf{H2}, we report statistical results of the performance metrics in terms of the interactive features by tasks. 




\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[width=\linewidth]{figures/taskCompletionTime-result-2024-2.png}
    \caption{
    The task completion time results by tasks, map types, and map layouts 
    % Accuracy comparison between single and multi-maps using static (left) and interactive (right) geospatial visualization. 
    % \placeholder{need to update}
    }
    \label{fig:single-multiple-performance-ci}
\end{figure}

% \begin{figure}[t]
%     \centering
%     % \setlength{\abovecaptionskip}{-3pt}
%     % \setlength{\belowcaptionskip}{-10pt}
%     \includegraphics[width=\linewidth]{figures/single-vs-multiple-dy.png}
%     \caption{\placeholder{need to update}Accuracy comparison between single and multi-maps using static (left) and interactive (right) geospatial visualization. 
%     % \placeholder{need to update}
%     }
%     \label{fig:single-multiple-performance-ci}
% \end{figure}




==> sections/Prev/8-discussion.tex <==
% diagnostic analysis in discussion section
\section{Discussion}

% \HDY{\textbf{In summary,} the results partially support \textbf{H1} and \textbf{H3}. We found that the accuracy could be significantly improved by the interactive features for five out of seven tasks (i.e., Associate, Categorize, Cluster, Identify, and Rank). However, no clear evidence that introduction of interactivity improves task accuracy for  Distinguish and Locate was found. 
% Next, we found multi-map is helpful for the Associate, Categorize, Cluster, Distinguish and Locate tasks. 
% However, single-map showed better performance in performing the Identify and Rank tasks compared to multi-map. 
% They suggest that the interactive map condition narrowed down the accuracy gaps to a slender margin between single and multi-map exploration.}

Our user study results partially support all hypotheses. 
In response to \textbf{RQ1}, we found that the results partially support \textbf{H1} and \textbf{H3}. The accuracy was significantly improved by the interactive features for five out of seven tasks (i.e., Associate, Categorize, Cluster, Identify, and Rank). These results align with the perspectives of both DiBiase \cite{dibiase1990visualization} and Roth \cite{roth2008addressing}, indicating that user interaction, particularly in terms of precision performance, aids in uncovering data relationships. However, we found no clear evidence that introducing interactivity improves task accuracy for Distinguish and Locate.  We also found that multi-map is helpful for the Associate, Categorize, Cluster, Distinguish and Locate tasks. 
However, single-map showed better performance in the Identify and Rank tasks compared to multi-map. 

Additionally, the results partially support \textbf{H2}. Despite the performance enhancements offered by the interactive features, we observed no noticeable variation in completion time for the Cluster and Rank tasks. However, the Associate, Categorize, and Identity tasks exhibited longer durations. 
In the following section, we explore RQ1 more thoroughly by examining the impact of participant expertise. We then proceed to analyze RQ2, drawing upon the insights gleaned from our study.



% In response to \textbf{RQ1}, the results indicate that the participants achieved greater accuracy using the interactive map compared to the traditional static contour map. 
% Table \ref{tab:task-wise-performance} shows that the interactive map condition improves the participants' accuracy in the associate, categorize, cluster, identify, and rank tasks, answering \textbf{RQ2}, while no statistical accuracy improvements in the distinguish and locate tasks are reported. 
% These results align with the perspectives of both DiBiase \cite{dibiase1990visualization} and Roth \cite{roth2008addressing}, indicating that user interaction, particularly in terms of precision performance, aids in uncovering data relationships. 
% In the following section, we explore RQ1 more thoroughly by examining the impact of participant expertise and proceed to analyze RQ2, drawing upon the insights gleaned from our study.
 





\subsection{Observations from the User Interaction Logs}
% We examine interaction logs from the perspectives of usage frequency, usage pattern over the task completion time, and usage sequence of each interactive feature. We discuss these observations in the context of the participating exploratory analysis task types. 
% To understand participants' interaction usage, pattern, and sequence, we classify the interactions based on the number of mouse/keyboard operations (steps) required to perform the feature.

% We examine interaction logs from the perspectives of usage frequency, usage pattern over the task completion time, and usage sequence of each interactive feature.
% We discuss these observations in the context of the participating exploratory analysis task types. 
To better understand participants' usage and pattern of interaction features, we examine interaction logs within the context of the exploratory analysis task types.
We classify the interactions based on the number of mouse/keyboard operations (steps) required to perform the feature. Following that, we eliminate unintended interactions in the process of aggregating their interaction logs.
For instance, despite participants only needing to move the cursor to inspect contour regions, they unintentionally interacted with other contour areas while navigating towards deeper parts of the map.
% For example, even though the participants only needed to move the cursor to inspect contour regions, they inadvertently interacted with other contour areas while navigating toward deeper parts of the map. % to reach the area laying deep inside the map border, the user interacts with other unintended contour regions as well. 
% To refine our findings, 
We filter out these unintended interactions by using a time threshold, focusing on areas where participants spent a notable duration, suggesting they were genuinely processing the information displayed on tooltips or widgets.
%. Hence, we determine the regions where participants spent reasonable time perceiving the information provided on the tooltip or widgets. 
Fig. \ref{fig:interaction-usage} shows a comprehensive overview of the usage patterns for the interactive features except for synchronization.
% across the 56 exploratory tasks (as distributed in Table \ref{tab:task-distribution}) executed by each participant. 


\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[width=\linewidth]{figures/interaction-usage-dy.png}
    \caption{
    The frequently used interactive features in the participating exploratory tasks. 
    % The four most frequently used interactive features in the participating ($t=56$) exploratory tasks. 
    % \placeholder{HDY: why 4? are we considering inspect and select as one same interactive feature?} 
    The plotted range of usage frequency is categorized by the task types and bootstrapped with a 95\% confidence interval.
    % \placeholder{HDY: what is t? how to read the figure?}
    }
    \label{fig:interaction-usage}
\end{figure}

\textbf{Identifying the frequently used interactive features:} 
% Upon analyzing participants' interaction behaviours using the interactive contour map, we found that the inspection and selection were the most frequently used functions, followed by annotation, filter/search, and controlling the contour styles. 
% Upon analyzing participants' interaction behaviors using the interactive contour map, 
We find that inspection and selection are the most frequently used functions, followed by annotation, filter/search, and encode. 
% From our analysis of the interaction logs, we note that 
First of all, we observe that the participants frequently inspected or selected various distinct contour regions during the tasks involving association, categorization, and clustering. We expect that they used these interactive features to understand the relationships among different intensity levels.
% \placeholder{TODO:This preference aligns with our expectations: the inspection and selection functions are a single-step interaction that displays basic information about the contour area. In contrast, other interactions such as search, annotation, and encoding involve multiple steps.}


Next, annotations are mostly used in the locate, rank, and associate tasks. 
% Annotations were mostly used in the tasks including locating, ranking, and associating, allowing participants to mark or inspect specific spatial data points. 
% These interactions include participants' self-made annotations and interaction with predefined markers on the maps. 
It is particularly useful in the rank task because the marker widget provides insights for comparison with other annotations, thereby aiding in determining the order of the contour regions. We also observe that the annotation interaction generally comes after the inspection, selection, and filter interactions.
% Annotations are particularly useful in the ranking tasks as the marker widget provides comparison insights with other annotations, hence, supports in deciding the order of the contour regions. We also observed that annotation interactions are generally performed followed by inspect/select and filter interactions.


The filter interaction is frequently utilized in the identify and categorize tasks, often involving searching based on geolocation. 
The identify tasks require to extract information based on geographical characteristics. Thus, participants used the search feature to annotate or inspect intensities according to the locations. The comparative information provided by the annotated locations is continuously updated as the participants interact with other contour regions providing effective categorization and clustering tasks, which involve identifying the regions with similar variability.


At last, we identify that the encoding feature is mostly used in the cluster and identify tasks. The contour encodings are understandably useful in the cluster tasks, as it is often required to identify the unique regions on the contour map. The identify tasks involve the geographical characteristics that usually reside in the base map, hence, the participants' controlled styles correlate with the contour map in these tasks. Therefore, changing the weight and opacity of the contour lines and region's area can be beneficial in visually performing these tasks.


\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[width=\linewidth]{figures/interaction-pattern-dy2.png}
    \caption{Task-wise user interaction pattern based on the normalized task completion time window. The highlighted area represents the time segments where participants' interactivity exceeds the mean.}
    \label{fig:interaction-pattern}
\end{figure}

\textbf{Reflecting cognitive process with interaction usage:}
% We closely observe the participants' interactive behaviors throughout each task's duration. 
% To better understand their foreseeable patterns, we normalized the task completion window and plotted user interactions (Fig. \ref{fig:interaction-pattern}). 
% To understand their foreseeable patterns, 
% We normalize the task completion window and plotted the number of user interaction usage as shown in Fig. \ref{fig:interaction-pattern}. 
% We normalize the task completion window and plotted the number of user interaction usage as shown in Fig. \ref{fig:interaction-pattern}. 
Fig. \ref{fig:interaction-pattern} presents the number of user interaction usage over time. We normalize the time based on task completion time for each task.
It provides the opportunity to estimate the segments where the participants are seemingly cognitively active. 
Red lines represent the average number of user interaction usage, and highlighted areas show the windows where participants' interactivity exceeds the average. 
The periods of inactivity, particularly at the beginning and end, reflect participants' cognitive processing as they attempted to comprehend the task at hand, plan their next move, or reach an analytical conclusion. 

% It is clear that periods of inactivity, particularly at the start and end, reflected participants' cognitive processing as they attempted to understand the task at hand and then reach an analytical conclusion. 
The average numbers of user interaction usage by the tasks reveal that the participants were especially interactive during more complex tasks such as associating, categorizing, and ranking. 
% \placeholder{\HDY{HDY: how do we know this?} 
They also devoted significant time to cognitively processing relationships between spatial data points.
% } 
In contrast, for tasks such as distinguishing and locating, participants were notably less interactive. 
% \placeholder{\HDY{HDY: how do we know this?}  
This pattern is further reflected in the accuracy score, where the performance disparity between static and interactive maps is minimal for these specific tasks.
% } %as the difference is insignificant between static and interactive maps in these task types.

% \paragraph*{\textbf{Perceiving the reasoning of interaction usage.} }
% From our analysis of the interaction logs, we note that the participants frequently inspected or selected various distinct contour regions before finalizing their decision.  
% The tasks such as associating, categorizing, and clustering require understanding the relationships among different intensity levels, which understandably prompted the participants to interact with the map repeatedly to reach analytical decisions.

% From our analysis of the interaction logs during complex tasks, we noted that participants frequently inspected or selected various distinct contour regions before finalizing their decision.
%t of distinct intensities, therefore, they reasonably interacted back and forth to reach an analytical decision. 

% Annotations are mostly used in the locate, rank, and associate tasks. 
% % Annotations were mostly used in the tasks including locating, ranking, and associating, allowing participants to mark or inspect specific spatial data points. 
% % These interactions include participants' self-made annotations and interaction with predefined markers on the maps. 
% It is particularly useful in the rank task because the marker widget provides insights for comparison with other annotations, thereby aiding in determining the order of the contour regions. We also observe that the annotation interaction generally comes after the inspection, selection, and filter interactions.
% % Annotations are particularly useful in the ranking tasks as the marker widget provides comparison insights with other annotations, hence, supports in deciding the order of the contour regions. We also observed that annotation interactions are generally performed followed by inspect/select and filter interactions.

% % \placeholder{[DY: i am not sure the context...]}
% The filter interaction is frequently utilized in the identify and categorize tasks, often involving searching based on geolocation. 
% The identify tasks require to extract information based on geographical characteristics. Thus, participants used the search feature to annotate or inspect intensities according to the locations. The comparative information provided by the annotated locations is continuously updated as the participants interact with other contour regions providing effective categorization and clustering tasks, which involve identifying the regions with similar variability.

% Encoding features are mostly used in cluster and identify tasks. The contour encodings are understandably useful in the cluster tasks, as it is often required to identify the unique regions on the contour map. The identify tasks involve the geographical characteristics that usually reside in the base map, hence, the participants' controlled styles correlate with the contour map in these tasks. Therefore, changing the weight and opacity of the contour lines and region's area can be beneficial in visually performing these tasks.

% \subsection{Interpretation of Results}
% \ic{add a discussion to compare our results with previous geo-visualization study results}

% We established two research questions to evaluate the usability of interactive contour maps in the seven types of exploratory analysis tasks under consideration. In response to \textbf{RQ1}, the results indicate that participants achieved greater accuracy using interactive contour maps compared to traditional static contours as shown in Fig. \ref{fig:overall-performance-error-plot}. Subsequently, we hypothesized that the interactive maps should reflect a significantly improved correctness score across the exploratory analysis task types. We also anticipated that participants would spend significantly more time with the interactive contour maps compared to the static maps. The ANOVA result (Table \ref{tab:task-wise-performance}) shows that participants' correctness scores in the associate, categorize, cluster, identify, and rank improved significantly (addressing \textbf{RQ2}). In contrast, improvements in the distinguish and locate-type tasks were statistically insignificant. Furthermore, the results show that participants took more time to perform tasks using the interactive maps, with notable differences in associate, categorize, and identify-type tasks are significant as shown in Fig. \ref{fig:performance-ci}.

% As the task distribution presented in Table \ref{tab:task-distribution}, we designed the repeated measures based on the spatial extent (\textit{short vs. long}), map layout (\textit{single vs. multi map}), geospatial expertise (\textit{novice vs. experienced}), task types (\textit{7 EDA}), and map interactivity (\textit{static vs. interactive}). Thus, we analyzed the fluctuations in participants' correctness scores accounting for these individual factors in interactive maps against static maps. We understand that the participants' correctness score difference in the static maps is significant between the single and multiple maps, especially for the associate, categorize, cluster, and rank-type tasks (Fig. \ref{fig:single-multiple-performance-ci}). In contrast, the score difference in the interactive maps between the single and multiple maps is statistically insignificant except for the locate and distinguish-type tasks. While we have not found any statistically significant interaction effect on the correctness score and the exploratory task types based on short versus long extent maps, our analysis shows evidence that the interactive mode brings the user performance close. We also measured user performance based on their reported geospatial expertise, considering both correctness score and completion time. While the experienced users consistently performed better than the novice users in both modes, the performance gaps are certainly closer between them in the interactive mode (Fig. \ref{fig:user-performance-by-expertise}), especially in complex tasks such as associate, cluster, and rank. 

% discuss master vs. novice
% effect of time-consuming interactions for instant tasks and observations queries..
% usability for exact value vs. estimated value tasks
% usage frequency of single-step vs multi-step user interacttions
% X -lack of user interaction in distinguish and locate resulted insignificant difference

% Quantitative evaluation in this study shares similarities with the previous studies \cite{koua2006, Herring2017, nagel2012} in terms of task design, participant recruitment, and analysis methods. However, the results from our experiments provide a unique understanding of the usability of the interactive features from different perspectives, as opposed to previous geovisual user studies, where only different visualization components \cite{koua2006}, display designs \cite{mahmood2019improving}, and visual stylization \cite{zahan2021contour} are evaluated for visual analysis tasks. Hence, this study provided scope to not only quantitatively measure participants' analytical performance but also their interaction behavior to report both descriptive and diagnostic analysis from the usage data. For instance, the analysis presented in Fig. \ref{fig:interaction-pattern} shows that participants least interacted in locate tasks where multi-step interactions are mostly utilized, thus, reflecting interaction behavior and potential reasoning for the insignificant performance difference against static maps. The result suggests that users' interactivity is inversely proportional to the number of steps required to perform the interaction.


\subsection{Performance Elevation by Geospatial Expertise}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/performance-by-user-expertise-dy.png}
    % \setlength{\abovecaptionskip}{-3pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Comparison between novice and experienced participants' performance suggests that novice users excel with interactive features significantly more than experienced users.
    \HDY{The X-axis represents user performance, measured as the total number of correct answers divided by the total task completion time.}
    }
    \label{fig:user-performance-by-expertise}
\end{figure*}


Our results show that the interactive map could improve the novice users' performance when compared to the static map, closing performance gaps between novice and experienced.
This is because interpreting information on a static map typically demands a certain level of expertise, whereas interactive maps have the potential to facilitate a better understanding for both expert and novice users alike. 
We examine the participants' accurate task completion per unit of time in the seven exploratory analysis task types. It is calculated by total number of correct answers by the total amount of task completion time. 
Fig. \ref{fig:user-performance-by-expertise} illustrates task-wise density plots to separately compare the performance measures of both novice and experienced users in interactive and static maps respectively. 
The dashed lines in Fig. \ref{fig:user-performance-by-expertise} represent the performance mean for static (gray) and interactive (green) maps. 
It shows that experienced users performed significantly better than novice users. 
It also shows that the interactive features improved novice users' performance in the associate, cluster, and rank tasks more than experienced users.
At the same time, however, the results reveal that the categorization task is found to be particularly difficult for novice users compared to the other tasks.

 \subsection{Design Considerations for Interactive Contour Map}
%\subsection{Summary of Findings}
% \rn{Based on the findings discussed, the following are suggested guidelines for visualization researchers focusing on contour-based geospatial visualization:}
\begin{itemize}
    \item \textbf{Prioritize Interactive Features:} Emphasize the development and improvement of interactive features.
    % including inspection, selection, annotation, filter/search, and encoding.
    Such features significantly influence users' analytical performance.

    \item \textbf{Consider User Expertise:} It is important to understand how performance varies with the expertise levels of end-users. Interactive maps can be particularly helpful for novice users, effectively bridging the performance gaps seen with traditional static maps.

    \item \textbf{Address Interaction Efficiency:} It is crucial to note that while interactive maps may improve accuracy, they might also increase task completion time. It is important to refine the efficiency of interactive features to ensure a balance between accuracy and time efficiency.

    \item \textbf{Tailor Interactions to Task Types:} 
    Interactive features should be customized based on the exploratory task types. For instance, emphasize inspection and selection for single-step interactions and consider multi-step interactions for tasks such as locating.
    % \item \rn{\textbf{Provide Data Annotations:} 
    In addition, the value of annotations, especially in tasks involving ranking and associating cannot be overstated. Users should be encouraged to engage with annotations after inspection, selection, and filter interactions to help their decision-making process.
    

    % \item \rn{\textbf{Understand Cognitive Processes:} Evaluating the interactive maps requires a deep reflection on the cognitive processes users engage in during different tasks. Recognize periods of inactivity may signify moments of cognitive processing and tailor interactive features to support users during these crucial phases.}
\end{itemize}

\subsection{Future Work}
% Despite the interactive features significantly improved the correctness in the geospatial data exploration tasks, the overall accuracy of visual estimation still requires further improvement, as shown in Fig. \ref{fig:overall-performance-error-plot}. 
In this work, we found that interactive features could significantly improve correctness in geospatial data exploration tasks. 
However, we observed that the participants struggled in complex exploratory tasks such as the associate, categorize, and cluster tasks which require in-depth spatial correlation and comparison compared to the simple identify and locate tasks.
Additionally, the overall correctness for the tasks is less than 70\%, indicating that the navigation task accuracy still needs to be improved.
% shows the overall correctness still below 70\% at best estimation. 
% We observed participants struggling in advanced exploratory tasks more than the simpler ones such as identify, and locate. Particularly in associate, categorize, and cluster types, the tasks where in-depth spatial correlation and comparison were required, participants achieved relatively lower correctness scores spending significantly more time than the other types of tasks as shown in Fig. \ref{fig:performance-ci}. 
% more than the simpler ones such as identify, and locate. 
% Particularly in associate, categorize, and cluster types, the tasks where in-depth spatial correlation and comparison were required, participants achieved relatively lower correctness scores spending significantly more time than the other types of tasks as shown in Fig. \ref{fig:performance-ci}. 
% Since the effect of interactive features is evident in the exploration visual analysis, there are plenty of scopes to implement advanced interactive features that facilitate these tasks. 
% \placeholder{Because the effect of interactive features is visible in the visual analysis of exploration, there are numerous opportunities to implement advanced interactive features that facilitate these tasks.}
Interactive features can effectively support users in data exploration beyond individual visualization elements by facilitating coordinated interactions among different visual components.
%we intend to formally survey the domain experts to outline the requirements for the interactive visual exploration of geospatial data. 
% While this study scrutinizes the interactions within the geospatial contour maps, the interacted features can be leveraged to coordinate multiple views to explore geospatial events \cite{Steed2020, nayeem2022dcpviz}. 
In our future research, we aim to investigate visualization components which could support the interactive map view and the benefits of coordinated interaction between them. 
% , as well as examining visualization components which could support the interactive map view. 
% For the spatiotemporal exploration, we intend to implement a multi-layer contour on a single map instance and design the user interaction for exploratory purposes. 
It also involves evaluating visualization approaches with various domain-specific experts in geographic spatial analysis, identifying their key tasks within each domain and evaluating interactive features that effectively support their tasks in terms of both quantitative and qualitative assessments.
% We also plan to include experts in geospatial analysis in both quantitative and qualitative evaluations of the interactive geospatial visualization. 
% While this study focused on temperature and precipitation intensity, representing both short and extensive spatial extent data, the insights gained will guide us in developing user interactions for more sophisticated analysis tasks.

% \placeholder{- performance in temperature vs precipitation map}

% \placeholder{- performance in the single vs multi map}

% \placeholder{- performance of somewhat* familiar vs expert participants}

% \placeholder{- }

% \subsection{Interaction Patterns}

% \subsection{Limitation \& Future Work}
% overall accuracy is poor
% multi map on top another for comparison

==> sections/Prev/9-conclusion.tex <==
\section{Conclusion}
In this work, we examined the usability of contour-based interactive geospatial visualization in exploratory analysis tasks.
% We implemented an interactive geospatial contour map and design a web-based interactive user study to quantitatively evaluate users' performance compared to the static geospatial map.
We implemented and designed \HDY{a} web interface and conducted \HDY{a} crowd-sourced user study to quantitatively evaluate and compare users' performance when using interactive and static geospatial maps. 
% We crowdsource the study and recruited 62 participants from Amazon MTurk for our experiment. 
% The interactive features are scrutinized against seven exploratory analysis tasks using temperature and precipitation contour maps. 
% The result suggests that the participants' task accuracy improved with the interactive maps, however, they needed additional time to complete the task compared to the static maps.
% The results suggest that task accuracy improved with the interactive maps while the participants took longer to complete the task than with static maps.
\HDY{The results suggest that using the interactive maps improved task accuracy but increases completion time compared to using the static maps.}
% task accuracy improved with the interactive maps, it took longer to complete the task than with static maps.
We also analyze participants' interaction logs to discuss the usability of the interactive features in the exploratory geospatial tasks. 
% Our findings can be used as guidelines for future visualization researchers and practioners to create use case-specific interactive geovisualizations for visually exploring geospatial data.
Our findings can be used as design considerations for future visualization researchers and practioners to create use case-specific interactive geovisualizations for visually exploring geospatial data.
% Our findings can serve as guidelines for visualization researchers in the future to develop use case-specific interactive geovisualization for visually exploring geospatial data.
